Making Generated Images Hard To Spot: A Transferable Attack On Synthetic Image Detectors

Visually realistic GAN-generated images have recently emerged as an important misinformation threat. Research has shown that these synthetic images contain forensic traces that are readily identifiable by forensic detectors. Unfortunately, these detectors are built upon neural networks, which are vulnerable to recently developed adversarial attacks. In this paper, we propose a new anti-forensic attack capable of fooling GAN-generated image detectors. Our attack uses an adversarially trained generator to synthesize traces that these detectors associate with real images. Furthermore, we propose a technique to train our attack so that it can achieve transferability, i.e. it can fool unknown CNNs that it was not explicitly trained against. We evaluate our attack through an extensive set of experiments, where we show that our attack can fool eight state-of-the-art detection CNNs with synthetic images created using seven different GANs, and outperform other alternative attacks.

==> sections/GenArchComp-Face-Full.tex <==
% GenArchComp-Face-Full.tex


\begin{table*}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
%\resizebox{.7\textwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|cc|cc|cc|}
\hline
%\multicolumn{7}{|c|}{\textbf{Proposed Adversarial Generator}}\\\hline\
 & \multicolumn{2}{|c|}{ Residual Gen.~\cite{residualgan}  } & \multicolumn{2}{|c|}{ MISLGAN~\cite{mislgan} } & \multicolumn{2}{|c|}{ CW } & \multicolumn{2}{|c|}{ FGSM }  & \multicolumn{2}{|c|}{ PGD }  & \multicolumn{2}{|c|}{ Proposed } \\\hline
\textbf{CNNs}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&{PSNR.}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&{PSNR.}&\textbf{ASR}&{PSNR.}&\textbf{ASR}&\textbf{PSNR}\\
\textbf{Xception}  & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000 &1.0000 &1.0000 &1.0000 &\textbf{1.0000}& 45.52&0.9875\\
\textbf{ResNet-50}  & 1.0000 &1.0000  & 1.0000 &1.0000 &1.0000 &1.0000  &  0.7590 & 0.8770& 0.8010 &\textbf{0.8123}&35.97 &0.9578\\
\textbf{DenseNet}  & 1.0000 &1.0000  & 1.0000 &1.0000 &1.0000 &1.0000 &0.9385 & 0.9770& 0.9970&\textbf{0.9708} &54.28&0.9997\\
\textbf{MISLNet}  & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000 & 0.9965  & 0.9905 &0.9950&\textbf{0.9940}&51.28 &0.9925\\
\textbf{PHNet}  & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000  &  1.0000&0.8497 &0.9985& \textbf{0.9494}&41.85&0.9753\\
\textbf{SRNet}   & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000 &  0.8080&0.8855 &0.9480&\textbf{0.8805}&50.97 &0.9922\\
\textbf{ImageCNN}  & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000  &  0.9854&0.9935 & 0.8505&\textbf{0.9431}&53.64 &0.9928\\
\textbf{CamID CNN}  & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000  &0.9285 &0.9120& 0.9870& \textbf{0.9425}& 58.10&0.9988\\ \hline
\textbf{Avg.}  & 1.0000 &1.0000 & 1.0000 &1.0000 &1.0000 &1.0000 &\textbf{0.9270}&\textbf{0.9357}&\textbf{0.9471}&\textbf{0.9366}&\textbf{48.95}&\textbf{0.9871}\\
\hline
\end{tabular}
%}
\label{tab: whiteboxface}
\end{table*}







%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%                       OLD                       %
%                                                     %
\begin{comment}

\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cccc||cc|}
\hline
%\multicolumn{7}{|c|}{\textbf{Proposed Adversarial Generator}}\\\hline
\multicolumn{4}{|c|c|c|c|}{& & &\textbf{Proposed}}\\\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} &1.0000 &1.0000 &1.0000 &\textbf{1.0000}& 45.52&0.9875\\
\textbf{ResNet-50} &  0.7590 & 0.8770& 0.8010 &\textbf{0.8123}&35.97 &0.9578\\
\textbf{DenseNet}&0.9385 & 0.9770& 0.9970&\textbf{0.9708} &54.28&0.9997\\
\textbf{MISLNet}& 0.9965  & 0.9905 &0.9950&\textbf{0.9940}&51.28 &0.9925\\
\textbf{PHNet} &  1.0000&0.8497 &0.9985& \textbf{0.9494}&41.85&0.9753\\
\textbf{SRNet} &  0.8080&0.8855 &0.9480&\textbf{0.8805}&50.97 &0.9922\\
\textbf{ImageCNN} &  0.9854&0.9935 & 0.8505&\textbf{0.9431}&53.64 &0.9928\\
\textbf{CamID CNN} &0.9285 &0.9120& 0.9870& \textbf{0.9425}& 58.10&0.9988\\
\textbf{Avg.}&\textbf{0.9270}&\textbf{0.9357}&\textbf{0.9471}&\textbf{0.9366}&\textbf{48.95}&\textbf{0.9871}\\
\hline

\multicolumn{7}{|c|}{\textbf{Residual Generator~\cite{residualgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception}& 0.9820&0.9940 &0.9770& 0.9843&29.01 &0.9498\\
\textbf{ResNet-50}& 0.1435 & 0.6010&0.5375&0.4273& 28.82&0.9448\\
\textbf{DenseNet}& 0.9915& 0.9955&0.9940 &0.9937& 29.72&0.9515\\
\textbf{MISLNet}&  0.9605&  0.9970&0.9880 & 0.9818&29.82& 0.9440\\
\textbf{PHNet} & 0.9665&0.9470 &0.9915 &0.9683 &30.21 &0.9556\\
\textbf{SRNet} &0.9605 & 0.9885& 0.9770&0.9753&29.46&0.9474\\
\textbf{Image CNN} & 1.0000&0.0000 & 1.0000&0.6667&29.21 &0.9531\\
\textbf{CamID CNN}& 0.9955& 0.9995&0.9990& 0.9980&28.89&0.9536\\
\textbf{Avg.} &0.8750&0.8150&0.9330&0.8744&29.39&0.9500\\

\hline
\multicolumn{7}{|c|}{\textbf{MISLGAN Generator~\cite{mislgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} & 1.0000& 0.0005& 1.0000&0.6668& 32.24&0.9598\\
\textbf{ResNet-50}& 0.4235&0.8115 & 0.7465&0.6605&34.64 &0.9630\\
\textbf{DenseNet}& 0.9995&1.0000 &0.9995 &0.9997 &35.11&0.9755\\
\textbf{MISLNet}& 0.9515 &  0.9965&0.9899 &0.9793 &34.50&0.9660 \\
\textbf{PHNet} & 0.9925& 0.9995 & 0.9985&0.9968&34.84 &0.9648\\
\textbf{SRNet} & 0.8915 & 0.9735&0.9635 &0.9428&33.09 &0.9550\\
\textbf{Image CNN} &0.7975 & 0.7980& 0.8205 &0.8053&34.36&0.9657\\
\textbf{CamID CNN}& 0.5410&0.3540 & 0.3720&0.4223& 33.30&0.9669\\
\textbf{Avg.} &0.8246&0.7417&0.8613&0.8092&34.01&0.9646\\
\hline
\end{tabular}}
\label{tab: whiteboxface}
\end{table}

\end{comment}

==> sections/GenArchComp-Face.tex <==
% GenArchComp-Face.tex


\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|}
\hline
%\multicolumn{7}{|c|}{\textbf{Proposed Adversarial Generator}}\\\hline\
 & \multicolumn{2}{|c|}{ Residual Gen.~\cite{residualgan}  } & \multicolumn{2}{|c|}{ MISLGAN~\cite{mislgan} } & \multicolumn{2}{|c|}{ Proposed } \\\hline
\textbf{CNNs}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&{PSNR.}&\textbf{ASR}&\textbf{PSNR}\\
\textbf{Xception} &1.0000 &1.0000 &1.0000 &\textbf{1.0000}& 45.52&0.9875\\
\textbf{ResNet-50} &  0.7590 & 0.8770& 0.8010 &\textbf{0.8123}&35.97 &0.9578\\
\textbf{DenseNet}&0.9385 & 0.9770& 0.9970&\textbf{0.9708} &54.28&0.9997\\
\textbf{MISLNet}& 0.9965  & 0.9905 &0.9950&\textbf{0.9940}&51.28 &0.9925\\
\textbf{PHNet} &  1.0000&0.8497 &0.9985& \textbf{0.9494}&41.85&0.9753\\
\textbf{SRNet} &  0.8080&0.8855 &0.9480&\textbf{0.8805}&50.97 &0.9922\\
\textbf{ImageCNN} &  0.9854&0.9935 & 0.8505&\textbf{0.9431}&53.64 &0.9928\\
\textbf{CamID CNN} &0.9285 &0.9120& 0.9870& \textbf{0.9425}& 58.10&0.9988\\
\textbf{Avg.}&\textbf{0.9270}&\textbf{0.9357}&\textbf{0.9471}&\textbf{0.9366}&\textbf{48.95}&\textbf{0.9871}\\
\hline
\end{tabular}}
\label{tab: whiteboxface}
\end{table}







%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%                       OLD                       %
%                                                     %
\begin{comment}

\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cccc||cc|}
\hline
%\multicolumn{7}{|c|}{\textbf{Proposed Adversarial Generator}}\\\hline
\multicolumn{4}{|c|c|c|c|}{& & &\textbf{Proposed}}\\\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} &1.0000 &1.0000 &1.0000 &\textbf{1.0000}& 45.52&0.9875\\
\textbf{ResNet-50} &  0.7590 & 0.8770& 0.8010 &\textbf{0.8123}&35.97 &0.9578\\
\textbf{DenseNet}&0.9385 & 0.9770& 0.9970&\textbf{0.9708} &54.28&0.9997\\
\textbf{MISLNet}& 0.9965  & 0.9905 &0.9950&\textbf{0.9940}&51.28 &0.9925\\
\textbf{PHNet} &  1.0000&0.8497 &0.9985& \textbf{0.9494}&41.85&0.9753\\
\textbf{SRNet} &  0.8080&0.8855 &0.9480&\textbf{0.8805}&50.97 &0.9922\\
\textbf{ImageCNN} &  0.9854&0.9935 & 0.8505&\textbf{0.9431}&53.64 &0.9928\\
\textbf{CamID CNN} &0.9285 &0.9120& 0.9870& \textbf{0.9425}& 58.10&0.9988\\
\textbf{Avg.}&\textbf{0.9270}&\textbf{0.9357}&\textbf{0.9471}&\textbf{0.9366}&\textbf{48.95}&\textbf{0.9871}\\
\hline

\multicolumn{7}{|c|}{\textbf{Residual Generator~\cite{residualgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception}& 0.9820&0.9940 &0.9770& 0.9843&29.01 &0.9498\\
\textbf{ResNet-50}& 0.1435 & 0.6010&0.5375&0.4273& 28.82&0.9448\\
\textbf{DenseNet}& 0.9915& 0.9955&0.9940 &0.9937& 29.72&0.9515\\
\textbf{MISLNet}&  0.9605&  0.9970&0.9880 & 0.9818&29.82& 0.9440\\
\textbf{PHNet} & 0.9665&0.9470 &0.9915 &0.9683 &30.21 &0.9556\\
\textbf{SRNet} &0.9605 & 0.9885& 0.9770&0.9753&29.46&0.9474\\
\textbf{Image CNN} & 1.0000&0.0000 & 1.0000&0.6667&29.21 &0.9531\\
\textbf{CamID CNN}& 0.9955& 0.9995&0.9990& 0.9980&28.89&0.9536\\
\textbf{Avg.} &0.8750&0.8150&0.9330&0.8744&29.39&0.9500\\

\hline
\multicolumn{7}{|c|}{\textbf{MISLGAN Generator~\cite{mislgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} & 1.0000& 0.0005& 1.0000&0.6668& 32.24&0.9598\\
\textbf{ResNet-50}& 0.4235&0.8115 & 0.7465&0.6605&34.64 &0.9630\\
\textbf{DenseNet}& 0.9995&1.0000 &0.9995 &0.9997 &35.11&0.9755\\
\textbf{MISLNet}& 0.9515 &  0.9965&0.9899 &0.9793 &34.50&0.9660 \\
\textbf{PHNet} & 0.9925& 0.9995 & 0.9985&0.9968&34.84 &0.9648\\
\textbf{SRNet} & 0.8915 & 0.9735&0.9635 &0.9428&33.09 &0.9550\\
\textbf{Image CNN} &0.7975 & 0.7980& 0.8205 &0.8053&34.36&0.9657\\
\textbf{CamID CNN}& 0.5410&0.3540 & 0.3720&0.4223& 33.30&0.9669\\
\textbf{Avg.} &0.8246&0.7417&0.8613&0.8092&34.01&0.9646\\
\hline
\end{tabular}}
\label{tab: whiteboxface}
\end{table}

\end{comment}

==> sections/WhiteBox-Face-Full.tex <==
% GenArchComp-Face-Full.tex

%\def\tablesize{0.7}

\begin{table*}[!t]
\centering
\label{tab: whiteboxface}
\caption{Mean attack success rates and mean image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{\tablesize\textwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{|c|}{ \textbf{Residual Gen.}~\cite{residualgan} } & \multicolumn{2}{|c|}{ \textbf{MISLGAN}~\cite{mislgan} } & \multicolumn{2}{|c|}{ \textbf{CW} } & \multicolumn{2}{|c|}{ \textbf{FGSM} }  & \multicolumn{2}{|c|}{ \textbf{PGD}}  & \multicolumn{2}{|c|}{ \textbf{Proposed}} \\\hline
\textbf{CNNs}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&{PSNR}&\textbf{ASR}&\textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}\\
\textbf{Xception}  & 0.9843 &29.01 & 0.6668  & 32.24&0.9848 &47.29 &0.5417 &44.20&1.0000&47.32 & 1.0000&45.52\\
\textbf{ResNet-50}  & 0.4273& 28.82& 0.6605 &34.64 &0.4091 &38.78 &  0.3750& 40.01 &0.5720  & 35.13&0.8123 &35.97\\
\textbf{DenseNet}  & 0.9937 &29.72 & 0.9997 & 35.11 &0.9432&50.36 &0.8750& 44.16& 0.9886&51.31 &0.9708 &54.28\\
\textbf{MISLNet}  & 0.9818 &29.82 & 0.9793 &34.50& 0.9546&50.53 & 0.5265 & 44.26 &1.0000&51.17&0.9940&51.28 \\
\textbf{PHNet}  & 0.9683 &30.21 & 0.9968 & 34.84 &0.9886&51.05 & 0.9773&51.14 &0.9924& 51.22&0.9494&41.85\\
\textbf{SRNet}   & 0.9753&29.46 & 0.9428  &33.09&0.9583&49.84 &  0.8187&51.14 &1.0000&51.22&0.8805 &50.97\\
\textbf{ImageCNN}  & 0.6667 &29.21 & 0.8050 &34.36 &1.0000 &49.54 & 0.0000&44.47 & 0.9470&49.04&0.9431&53.64 \\
\textbf{CamID CNN}  & 0.9980 &28.89& 0.4223 &33.30&0.9469 &49.25  &0.0038 &44.16 & 0.9288&51.15 &0.9425& 58.10\\ \hline
\textbf{Avg.}  & 0.8744 &29.39& 0.8092 &34.01 &0.8982&48.33&0.5147&0.4544 &0.9286 &48.44 & \textbf{0.9366}&\textbf{48.95}\\
\hline
\end{tabular}
}
\end{table*}







%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%                       OLD                       %
%                                                     %
\begin{comment}
\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cccc||cc|}
\hline
%\multicolumn{7}{|c|}{\textbf{Proposed Adversarial Generator}}\\\hline
\multicolumn{4}{|c|c|c|c|}{& & &\textbf{Proposed}}\\\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} &1.0000 &1.0000 &1.0000 &\textbf{1.0000}& 45.52&0.9875\\
\textbf{ResNet-50} &  0.7590 & 0.8770& 0.8010 &\textbf{0.8123}&35.97 &0.9578\\
\textbf{DenseNet}&0.9385 & 0.9770& 0.9970&\textbf{0.9708} &54.28&0.9997\\
\textbf{MISLNet}& 0.9965  & 0.9905 &0.9950&\textbf{0.9940}&51.28 &0.9925\\
\textbf{PHNet} &  1.0000&0.8497 &0.9985& \textbf{0.9494}&41.85&0.9753\\
\textbf{SRNet} &  0.8080&0.8855 &0.9480&\textbf{0.8805}&50.97 &0.9922\\
\textbf{ImageCNN} &  0.9854&0.9935 & 0.8505&\textbf{0.9431}&53.64 &0.9928\\
\textbf{CamID CNN} &0.9285 &0.9120& 0.9870& \textbf{0.9425}& 58.10&0.9988\\
\textbf{Avg.}&\textbf{0.9270}&\textbf{0.9357}&\textbf{0.9471}&\textbf{0.9366}&\textbf{48.95}&\textbf{0.9871}\\
\hline

\multicolumn{7}{|c|}{\textbf{Residual Generator~\cite{residualgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception}& 0.9820&0.9940 &0.9770& 0.9843&29.01 &0.9498\\
\textbf{ResNet-50}& 0.1435 & 0.6010&0.5375&0.4273& 28.82&0.9448\\
\textbf{DenseNet}& 0.9915& 0.9955&0.9940 &0.9937& 29.72&0.9515\\
\textbf{MISLNet}&  0.9605&  0.9970&0.9880 & 0.9818&29.82& 0.9440\\
\textbf{PHNet} & 0.9665&0.9470 &0.9915 &0.9683 &30.21 &0.9556\\
\textbf{SRNet} &0.9605 & 0.9885& 0.9770&0.9753&29.46&0.9474\\
\textbf{Image CNN} & 1.0000&0.0000 & 1.0000&0.6667&29.21 &0.9531\\
\textbf{CamID CNN}& 0.9955& 0.9995&0.9990& 0.9980&28.89&0.9536\\
\textbf{Avg.} &0.8750&0.8150&0.9330&0.8744&29.39&0.9500\\

\hline
\multicolumn{7}{|c|}{\textbf{MISLGAN Generator~\cite{mislgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} & 1.0000& 0.0005& 1.0000&0.6668& 32.24&0.9598\\
\textbf{ResNet-50}& 0.4235&0.8115 & 0.7465&0.6605&34.64 &0.9630\\
\textbf{DenseNet}& 0.9995&1.0000 &0.9995 &0.9997 &35.11&0.9755\\
\textbf{MISLNet}& 0.9515 &  0.9965&0.9899 &0.9793 &34.50&0.9660 \\
\textbf{PHNet} & 0.9925& 0.9995 & 0.9985&0.9968&34.84 &0.9648\\
\textbf{SRNet} & 0.8915 & 0.9735&0.9635 &0.9428&33.09 &0.9550\\
\textbf{Image CNN} &0.7975 & 0.7980& 0.8205 &0.8053&34.36&0.9657\\
\textbf{CamID CNN}& 0.5410&0.3540 & 0.3720&0.4223& 33.30&0.9669\\
\textbf{Avg.} &0.8246&0.7417&0.8613&0.8092&34.01&0.9646\\
\hline
\end{tabular}}
\end{table}
\end{comment}

==> sections/WhiteBox-Object-Full.tex <==
% GenArchComp-Face-Full.tex

\begin{table*}[!t]
\label{tab: whiteboxobject}
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Mean attack success rates and mean image quality achieved for white-box attacks on the Object Dataset.}
\resizebox{\tablesize\textwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{|c|}{ \textbf{Residual Gen.}~\cite{residualgan} } & \multicolumn{2}{|c|}{ \textbf{MISLGAN}~\cite{mislgan} } & \multicolumn{2}{|c|}{ \textbf{CW} } & \multicolumn{2}{|c|}{ \textbf{FGSM} }  & \multicolumn{2}{|c|}{ \textbf{PGD}}  & \multicolumn{2}{|c|}{ \textbf{Proposed}} \\\hline
\textbf{CNNs}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&{PSNR}&\textbf{ASR}&\textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}\\
\textbf{Xception} & 0.9963&39.73 &0.9483&32.09 &0.6667&50.31 &0.7482 &51.19&0.6742&51.15 & 0.9952&52.59\\
\textbf{ResNet-50} &0.9461&38.51 &0.8846& 31.50& 0.8985&49.58  &  0.7479& 51.16& 0.8636& 51.17&0.9524&55.41\\
\textbf{DenseNet}  &0.9522&37.52 &0.9515&31.22 &0.8123 &50.80 &0.7993 & 51.15& 0.8181 &51.16&0.9116&50.22\\
\textbf{MISLNet} &0.8353&40.49 &0.9912&31.75 & 0.6402&51.08 & 0.6591 & 51.26 &0.7121&51.16&0.9270&50.97\\
\textbf{PHNet} & 0.9646&40.22 & 0.8307&31.00 &0.8220 &50.93 &  0.8182&51.15 &0.8371&51.15 & 0.9802&51.99\\
\textbf{SRNet}  &0.8206&37.36 & 0.9406&31.68 &0.6135 & 46.61& 0.0000 &51.16 &0.7235&51.15  &0.8287&56.41\\
\textbf{ImageCNN}  & 0.6342&38.66 &0.8109 & 33.43 &0.6705 &50.95 &0.6970  &51.46& 0.6932&51.15 &0.8057&55.32 \\
\textbf{CamID CNN}  &0.8039&39.02 &0.7569& 31.37 &0.6061&49.01&0.5909&51.34 & 0.5720& 51.15&0.9305&52.77\\ \hline
\textbf{Avg.}  &0.8695&38.94 &0.8893&31.76 &0.7162&49.91 &0.6319&51.23&0.7367&51.16&\textbf{0.9164}&\textbf{53.21}\\
\hline
\end{tabular}
}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%                       OLD                       %
%                                                     %
\begin{comment}
\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of objects in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Object Dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|ccccccc||cc|}
\hline
\multicolumn{10}{|c|}{\textbf{Proposed Adversarial Generator}}\\
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM}\\
\textbf{Xception} &0.9880 &0.9871 &0.9995 & 1.0000 & 0.9975& 0.9992&\textbf{0.9952}&52.59&0.9972 \\
\textbf{ResNet-50} &0.9174 &0.8720 & 0.9910& 0.9971& 0.9520&0.9848 &\textbf{0.9524}&55.41&0.9973 \\
\textbf{DenseNet}  & 0.8583&0.8432 &0.9457 & 0.9474&0.9350 & 0.9402&\textbf{0.9116}&50.22&0.9893\\
\textbf{MISLNet} & 0.9437& 0.6409& 0.9893& 0.9954&0.9930&0.9994&\textbf{0.9270}&50.97&0.9925 \\
\textbf{PHNet}  & 0.9645 &0.9477 &0.9834 & 0.9985& 0.9890& 0.9978& \textbf{0.9802}&51.99&0.9613\\
\textbf{SRNet} & 0.7980 & 0.5758 & 0.9577& 0.9959& 0.7600& 0.8846&\textbf{0.8287}&56.41&0.9940\\
\textbf{Image CNN} &0.6890 & 0.6644 & 0.9341&0.9772  &0.8540 & 0.7152&\textbf{0.8057}&55.32&0.9981\\
\textbf{CamID CNN} & 0.8650 &0.8470 & 0.9694&0.9622 & 0.9445& 0.9946&\textbf{0.9305}&52.77 &0.9970\\
\textbf{Avg.} &\textbf{0.8780}&\textbf{0.7973}&\textbf{0.9713}&\textbf{0.9842}&\textbf{0.9281}&\textbf{0.9395}&\textbf{0.9164}&\textbf{53.21}&\textbf{0.9908}\\
\hline
\multicolumn{10}{|c|}{\textbf{Residual Generator~\cite{residualgan}}}\\
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.} &\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM} \\
\textbf{Xception} &0.9927 &0.9954 &0.9983 & 0.9936 & 0.9975 & 1.0000 &0.9963&39.73&0.9612 \\
\textbf{ResNet-50} &0.9197    &0.9447 & 0.9376& 0.9588 & 0.9490 & 0.9670&0.9461&38.51&0.9728\\
\textbf{DenseNet}  &0.9582 & 0.9242&0.9677 & 0.9724&0.9585 & 0.9322&0.9522&37.52&0.9543\\
\textbf{MISLNet} & 0.7800 & 0.6068& 0.7952& 0.9644& 0.8910 & 0.9934&0.8353&40.49&0.9875 \\
\textbf{PHNet}  & 0.9287 &0.9758 &0.9405 & 0.9766 & 0.9745& 0.9916& 0.9646&40.22&0.9719\\
\textbf{SRNet} & 0.7215&0.6485 &0.8590  &0.9658  &0.8180 &0.9110 &0.8206&37.36&0.9649\\
\textbf{Image CNN} &0.6580 &  0.6114 & 0.7811 & 0.9543 &0.5905 & 0.2096& 0.6342&38.66&0.9679\\
\textbf{CamID CNN} & 0.6207 &0.6121 & 0.8789&0.9669 &0.8860 & 0.8590&0.8039&39.02 &0.9736\\
\textbf{Avg.} &0.8224&0.7899&0.8949&0.9691&0.8831&0.8580&0.8695&38.94&0.9693\\
\hline
\multicolumn{10}{|c|}{\textbf{MISLGAN Generator~\cite{mislgan}}}\\
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.} &\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM} \\
\textbf{Xception} &0.9405 & 0.9477& 0.9666&  0.9783&0.9155 & 0.9414&0.9483&32.09&0.9651 \\
\textbf{ResNet-50} & 0.9117&0.8955 & 0.9025& 0.7645& 0.9614& 0.8720&0.8846& 31.50&0.9547\\
\textbf{DenseNet}  &0.9687 & 0.9227 & 0.9674& 0.9772& 0.9300& 0.9432&0.9515&31.22&0.8470\\
\textbf{MISLNet} &0.9905 & 0.9905 &0.9915 &0.9880 &0.9910  &0.9955 &0.9912&31.75& 0.9602\\
\textbf{PHNet}  & 0.8200&0.8465 & 0.8215&0.8250 &0.8305  &0.8405 & 0.8307&31.00&0.9495 \\
\textbf{SRNet} & 0.9230 & 0.8114 & 0.9719& 0.9979&  0.9495&0.9896 & 0.9406&31.68& 0.9689\\
\textbf{Image CNN} & 0.7333& 0.7205  & 0.8879& 0.9866 & 0.8000& 0.7368&0.8109 & 33.43&0.8750\\
\textbf{CamID CNN} &  0.6925& 0.6636& 0.7821& 0.9417& 0.6995&0.7618 &0.7569& 31.37&0.9120\\
\textbf{Avg.} &0.8725&0.8498&0.9114&0.9324&0.8847&0.8851&0.8893&31.76&0.9291\\
\hline
\end{tabular}}
\label{tab: whiteboxobject}
\end{table}

\end{comment}

==> sections/Zero-Face-Full.tex <==
% GenArchComp-Face-Full.tex

\begin{table*}[!t]
\label{tab: zeroface}
\centering
\caption{Mean attack success rates and mean image quality achieved for  zero-knowledge attacks on the Human Face Dataset. }
%\resizebox{\tablesize\textwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{|c|}{\textbf{CW}} & \multicolumn{2}{|c|}{\textbf{FGSM}}  & \multicolumn{2}{|c|}{\textbf{PGD}}  & \multicolumn{2}{|c|}{ \textbf{Proposed}} \\\hline
\textbf{CNNs}& \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}&\textbf{ASR}&\textbf{PSNR}\\
\textbf{Xception}  & 0.1975 &39.58&0.1758 &40.07&0.0054&38.89& 0.9107 &37.93\\
\textbf{ResNet-50}  &0.1953 &39.99  &  0.2018 & 40.07 & 0.1813 &38.15&0.2435 & 42.90\\
\textbf{DenseNet}   &0.1272 &39.97 &0.0406 &40.07 &0.0487&38.92& 0.8730&38.79\\
\textbf{MISLNet}  &0.0050 &39.91 & 0.0000 & 40.06 &0.0005&38.89&0.3980 &38.14\\
\textbf{PHNet} &0.0422&40.18 & 0.0008&40.07 &0.1461& 38.98&0.9162&41.69\\
\textbf{SRNet}    & 0.1191&  39.72&0.1645 &40.07&0.0108&38.98&0.8878 &40.16\\
\textbf{ImageCNN}  &0.1109&39.55 &  0.1169&40.03& 0.1477&38.87&0.8673&41.27 \\
\textbf{CamID CNN}  &0.0005 &39.84  &0.0000&40.07& 0.1082& 38.92& 0.9117 &42.77\\ \hline
\textbf{Avg.} & 0.0997 &39.84&0.0885&40.06&0.0647&38.84&\textbf{0.7510}&\textbf{40.46}\\
\hline
\end{tabular}
%}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%                       OLD                       %
%                                                     %
\begin{comment}
\begin{table}[!t]
\centering
%\caption{Evaluation of the proposed attack against the victim CNN for detecting GAN-generated images of human faces in the zero knowledge scenario. }
\caption{Attack success rates and image quality achieved for zero-knowledge attacks on the Human Face Dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cccc||cc|}
\hline
 \textbf{CNNs} & \textbf{StarGAN-v2}&\textbf{StyleGAN}& \textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} &0.7855 &0.9565& 0.9900 &\textbf{0.9107} &37.93  &0.9766\\
\textbf{ResNet-50}  &0.0695  & 0.3795 &0.2815 &\textbf{0.2435}& 42.90 &0.9765 \\
\textbf{DenseNet} &  0.8345 & 0.8325&0.9520 &\textbf{ 0.8730}&38.79 & 0.9480\\
\textbf{MISLNet} &  0.1250 &  0.2340 & 0.8350 & \textbf{0.3980} &38.14&0.9742\\
\textbf{PHNet} &0.9925 & 0.7625 &0.9935 &\textbf{0.9162}&41.69& 0.9704\\
\textbf{SRNet} &  0.8495 & 0.8675  &0.9465 &\textbf{0.8878} &40.16 &0.9709\\
\textbf{Image CNN} & 0.8360 &0.9595& 0.8065 &\textbf{0.8673}&41.27 &0.9590 \\
\textbf{CamID CNN} &  0.7990& 0.9480 &0.9880 &\textbf{0.9117} &42.77&0.9703 \\
\textbf{Avg.}&\textbf{0.6614}& \textbf{0.7425}&\textbf{0.8491}& \textbf{0.7510}&\textbf{40.46}&\textbf{0.9682}\\
\hline
\end{tabular}}
\label{tab: zeroface}
\end{table}
\end{comment}





==> sections/Zero-Object-Full.tex <==
% GenArchComp-object-Full.tex

\begin{table*}[!t]
\centering
\label{tab: zeroobject}
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Mean attack success rates and mean image quality achieved for zero-knowledge attacks on the Object Dataset. }
%\resizebox{\tablesize\textwidth}{!}{
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{|c|}{\textbf{CW}} & \multicolumn{2}{|c|}{\textbf{FGSM}}  & \multicolumn{2}{|c|}{\textbf{PGD}}  & \multicolumn{2}{|c|}{ \textbf{Proposed}} \\\hline
\textbf{CNNs}&  \textbf{ASR} & \textbf{PSNR}&\textbf{ASR}&{PSNR.}&\textbf{ASR}&{PSNR.}&\textbf{ASR}&\textbf{PSNR}\\
\textbf{Xception}  & 0.4570 &40.95&0.4167 &40.12 &1.0000 &\textbf{1.0000}& \textbf{0.9663}&39.95\\
\textbf{ResNet-50}  &0.7020 & 41.09& 0.5043 & 40.13& 0.8010 &\textbf{0.8123}&\textbf{0.8045}& 41.75\\
\textbf{DenseNet}   &0.6874&41.17&0.5271& 40.13& 0.9970&\textbf{0.9708} &\textbf{0.9519}&40.46\\
\textbf{MISLNet}  &0.4337 &41.63 & 0.5292& 40.11 &0.9950&\textbf{0.9940}&\textbf{0.2504 }&41.39 \\
\textbf{PHNet} &0.5146 &41.38  & 0.4167& 40.13 &0.9985& \textbf{0.9494}&\textbf{0.9748}&42.18\\
\textbf{SRNet}    &0.1173 &41.25& 0.1645& 40.13 &0.9480&\textbf{0.8805}&\textbf{0.0849}& 39.95\\
\textbf{ImageCNN}  &0.3934&41.20  &  0.5297&40.02& 0.8505&\textbf{0.9431}&\textbf{0.6038}& 41.03\\
\textbf{CamID CNN}  &0.5270&40.82  &0.5357&40.09& 0.9870& \textbf{0.9425}& \textbf{0.9906}&43.43\\ \hline
\textbf{Avg.}  & 0.5270 &41.19 &0.4530&40.11&\textbf{0.9471}&\textbf{0.9366}&\textbf{0.7030}&\textbf{41.27}\\
\hline
\end{tabular}
%}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%                       OLD                       %
%                                                     %
\begin{comment}
\begin{table}[!t]
\centering
%\caption{Evaluation of the proposed attack against the victim CNNs for detecting GAN-generated images of objects in the zero knowledge scenario. }
\caption{Attack success rates and image quality achieved for zero-knowledge attacks on the Object Dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|ccccccc||cc|}
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM}\\
\textbf{Xception} &0.9215&0.9568 &0.9811&0.9986&0.9525& 0.9684& \textbf{0.9663}&39.95&0.9510\\
\textbf{ResNet-50} &0.7022&0.7742 &0.7798 &0.7816 & 0.8990 &0.8902&\textbf{0.8045}& 41.75&0.9628 \\
\textbf{DenseNet} & 0.9692& 0.9508& 0.9712 &0.8922 &0.9540 & 0.9740 &\textbf{0.9519}&40.46&0.9214 \\
\textbf{MISLNet} &0.1163 &0.1318 & 0.1264& 0.1325&  0.3035 & 0.6920&\textbf{0.2504 }&41.39 &0.9353\\
\textbf{PHNet} &0.9525&0.9652& 0.9796&0.9959 &0.9669& 0.9888&\textbf{0.9748}&42.18 &0.9417 \\
\textbf{SRNet} &0.0223 & 0.0000 & 0.2483& 0.2359& 0.0010& 0.0020&\textbf{0.0849}& 39.95&0.9510\\
\textbf{Image CNN} & 0.6515 & 0.6136 &0.8462 & 0.9238&  0.4840& 0.1036 &\textbf{0.6038}& 41.03& 0.9653 \\
\textbf{CamID CNN} & 0.9885&0.9561 & 0.9997& 0.9990 &1.0000&1.0000 & \textbf{0.9906}&43.43&0.9361 \\
\textbf{Avg.}&\textbf{0.6655}&\textbf{0.6686}& \textbf{0.7415}&\textbf{0.7449}& \textbf{0.6961}&\textbf{0.7024}&\textbf{0.7030}&\textbf{41.27}&\textbf{0.9456}\\
\hline
\end{tabular}}
\end{table}
\end{comment}




==> sections/background.tex <==
%background
\section{Related Work}

\subsection{GAN-generated Image Detectors}
Synthesized  objects and human faces pose a great threat to media securities~\cite{starganv2choi2020, stylegan2Karras2019, stylegankarras2019style,  bigganbrock2018large,gauganpark2019gaugan,progankarras2017progressive,  choi2018stargan}.  Generative adversarial networks (GANs)~\cite{GAN2014} based techinques  are one of the most popular approaches and show strong performances in synthesizing visually plausible human faces,  such as the StyleGAN, StyleGAN2~\cite{stylegankarras2019style,  stylegan2Karras2019}.  To combat with the synthesized images,   much research in computer vision community and multimedia forensics community has been done to to  address the problem of detecting GAN synthesized  images~\cite{9010964,  8397040, cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn}.   Previous  research shown that GANs left behind forensic traces that are very distinguishable from real images.  These forensic traces left by GANs can be utilized to detect GAN-generated images~\cite{cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn},  or identify which GAN was used to generate the images~\cite{marra2018gans,  9010964}.  

Recently Wang et al.~\cite{wang2020cnn} showed that by CNNs can be trained  to learn  general forensic traces  left by synthesized images (mostly by GANs).  Therefore,  by training a binary classifier between real and synthesized images produced by one GAN method. The trained classifier  can be used to  detect other synthesized images produced by other methods.  The author used  ResNet-50~\cite{resnet} pretrained on ImageNet~\cite{imagenet},  and trained it to distinguish between real and ProGAN generated  fake  images,  and then showed that  the  ResNet-50 detector can detect generated images produced by other generative methods unseen by the detector during training,  including  six popular GAN methods. 

\subsection{Adversarial Attacks on Forensic Classifiers}
At the same time,  the countermeasures against the CNN detectors for synthesized images  have arisen.   The main goal of the adversarial attacks on CNN detectors  is to make the CNNs classify the images after the attack as ``real".  The two families of  adversarial attacks on  CNN classifiers are adversarial example-based attacks~\cite{L-BFGS,  cw,   fgsm,  iterative-fg, deepfool, pgd, brown2017adversarial} and GAN-based attacks~\cite{mislgan,  poursaeed2018generative,  baluja2017adversarial, residualgan}. 

\subhead{Adversarial example-based attacks} Many adversarial attacks operates by adding perturbations to images to cause CNN to misclassify,  such as L-BFGS~\cite{L-BFGS},  FGSM and iterative-FG~\cite{fgsm,iterative-fg},  JSMA~\cite{jsma},  CW~\cite{cw},  PGD~\cite{pgd},  Most of the existing adversarial attacks on CNNs operate by adding noises to an image to cause the CNN to misclassify.    The noises is image dependent, 

\subhead{GAN-based attacks} Previous research also show that 

==> sections/background_v2.tex <==
%background
\section{Related Work}

Here we briefly review related work on detecting {\gi}s and adversarial attacks against forensic classifiers.

\subhead{GAN-Generated Image Detectors}
%Synthesized  objects and human faces pose a great threat to media securities~\cite{starganv2choi2020, stylegan2Karras2019, stylegankarras2019style,  bigganbrock2018large, gauganpark2019gaugan, progankarras2017progressive,  choi2018stargan}.  Generative adversarial networks (GANs)~\cite{GAN2014} based techinques  are one of the most popular approaches and show strong performances in synthesizing visually plausible human faces,  such as the StyleGAN, StyleGAN2~\cite{stylegankarras2019style,  stylegan2Karras2019}.  
%
To combat with the synthesized images,  much research in computer vision community and multimedia forensics community has been done to to  address the problem of detecting GAN synthesized  images~\cite{9010964,  8397040, cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn}.   Previous  research shown that GANs left behind forensic traces that are very distinguishable from real images.  These forensic traces left by GANs can be utilized to detect GAN-generated images~\cite{cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn},  or identify which GAN was used to generate the images~\cite{marra2018gans,  9010964}.  

%Recently Wang et al.~\cite{wang2020cnn} showed that by CNNs can be trained  to learn  general forensic traces  left by synthesized images (mostly by GANs).  Therefore,  by training a binary classifier between real and synthesized images produced by one GAN method. The trained classifier  can be used to  detect other synthesized images produced by other methods.  The author used  ResNet-50~\cite{resnet} pretrained on ImageNet~\cite{imagenet},  and trained it to distinguish between real and ProGAN generated  fake  images,  and then showed that  the  ResNet-50 detector can detect generated images produced by other generative methods unseen by the detector during training,  including  six popular GAN methods. 


\subhead{Adversarial Attacks on Forensic Classifiers}
%
At the same time,  the countermeasures against the CNN detectors for synthesized images  have arisen.   The main goal of the adversarial attacks on CNN detectors  is to make the CNNs classify the images after the attack as ``real".  The two families of  adversarial attacks on  CNN classifiers are adversarial example-based attacks~\cite{L-BFGS,  cw,   fgsm,  iterative-fg, deepfool, pgd, brown2017adversarial} and GAN-based attacks~\cite{mislgan,  poursaeed2018generative,  baluja2017adversarial, residualgan}. 

\subhead{Adversarial example-based attacks} Many adversarial attacks operates by adding perturbations to images to cause CNN to misclassify,  such as L-BFGS~\cite{L-BFGS},  FGSM and iterative-FG~\cite{fgsm,iterative-fg},  JSMA~\cite{jsma},  CW~\cite{cw},  PGD~\cite{pgd},  Most of the existing adversarial attacks on CNNs operate by adding noises to an image to cause the CNN to misclassify.    The noises is image dependent, 

\subhead{GAN-based attacks} Previous research also show that 

==> sections/difference_from_adv_examples.tex <==
% difference_from_adv_examples



We note that this attack is different from adversarial example generation algorithms % developed in machine learning literature  
such as FGSM, PGD, or CW~\cite{ } in several important ways.  

These algorithms all approximately operate by creating pertubations $\delta$ that are added to an image in order to fool a classifier.  The adversarial perturbations $\delta$ are the same size as the input to the victim classifier.  %, and are iteratively learned by 
They are learned through an iterative process in which an intermediate version of the attacked image is presented to the victim classifier, gradient information is inferred, and the attack perturbation is updated.  As a result, a new perturbation must be iteratively learned for each image under attack.

By contrast our attack learns a convolutional generator which is trained in advance.   The generator is not modified or customized to the image under attack.   Any image of arbitrary size can be passed through the generator, not just images with the same size as the victim CNN's input.  

Most importantly, our attack differs philosophically from adversarial examples.  Adversarial examples aim to find minor perturbations that cause a victim classifier to misclassify an input.  Several explanations as to why adversarial examples exist, including 
imperfections caused by the locally-linear nature of neural networks 
%% [11] - Goodfellow, Ian J., Jonathon Shlens, and Christian Szegedy. "Explaining and harnessing adversarial examples." arXiv preprint arXiv:1412.6572 (2014).
or that there is misalignment between the features used by humans and those learned by neural networks when performing the same classification task.
% Adversarial Examples Are Not Bugs, They Are Features
%
%  They accomplish this goal by exploiting ``blind spots'' that occur due to %inadequate training or overfitting to t

Our attack instead aims to accurately synthesize forensic features used by a CNN, that are otherwise used to \textit{correctly} classify that image.  


Our attack does intend to exploit adversarial perturbations that may clause a neural network to misclassify an input.  Instead, our attack aims to accurately synthesize the forensic features that are used are used to \textit{correctly} classify an unattacked image. 
%
When doing this, we are able to exploit the fact that forensic traces are not visible to the human eye.  As a result, we can completely falsify these traces without modifying the contents of an image.  We believe that this is the key to the improved transferability of our attack.  
%We note, however, that this approach may not work against classifiers for computer vision tasks because 

%This approach may not be possible 








%%%%%%%% WRITING NOTE %%%%%%%%
%From Carlini & Wagner, "Towards Evaluating the Robustness of Neural Networks"
%The key insight here is that by training to match the first network, we will hopefully avoid over-fitting against any of the training data. If the reason that neural networks exist is because neural networks are highly non-linear and have “blind spots” [46] where adversarial examples lie, then preventing this type of over-fitting might remove those blind spots.
%
% REFERENCE [46] - SZEGEDY, C., ZAREMBA, W., SUTSKEVER, I., BRUNA, J., ERHAN, D., GOODFELLOW, I., AND FERGUS, R. Intriguing properties of neural networks. ICLR (2013).
%
%
% IIn fact, as we will see later, defensive distillation does not remove adversarial examples. One potential reason this may occur is that others [11] have argued the reason adversarial examples exist is not due to blind spots in a highly non-linear neural network, but due only to the locally-linear nature of neural networks. This so-called linearity hypothesis appears to be true [47], and under this explanation it is perhaps less surprising that distillation does not increase the robustness of neural network
%
% [11] - Goodfellow, Ian J., Jonathon Shlens, and Christian Szegedy. "Explaining and harnessing adversarial examples." arXiv preprint arXiv:1412.6572 (2014).

% Adversarial Examples Are Not Bugs, They Are Features




==> sections/difference_from_adv_examples_v2.tex <==
% difference_from_adv_examples_v2


\begin{comment}
%This
%Our proposed attack, as well as other GAN-based attacks,  are 
Our proposed attack is 
different from adversarial example generation algorithms % developed in machine learning literature  
such as FGSM, PGD, or CW~\cite{fgsm, pgd, cw} 
in several important ways.  
\end{comment}

Our proposed attack is 
different from adversarial example generation algorithms 
in several %important 
ways.  
%
Most importantly, our attack operates using a fundamentally different  approach than adversarial examples.  
%differs from adversarial examples in the way which it works. 
 Adversarial examples aim to exploit non-ideal properties neural networks that can cause them to misclassify an input image.  % in a desired fashion.  
Several explanations have been posited for the non-ideal properties of neural networks that adversarial examples exploit,  such as 
imperfections caused by the locally-linear nature of neural networks~\cite{fgsm} %,  
%``blind spots'' caused by non-ideal training or overfitting~\cite{ }, 
or that there is misalignment between the features used by humans and those learned by neural networks when performing the same classification task~\cite{ilyas2019adversarial}.



%%%%%
%
\begin{comment}
Most importantly,  the underlying philosophy %goal 
of our attack differs from that of adversarial examples.  Adversarial examples aim to find minor perturbations that cause a victim classifier to misclassify an input image.  Several explanations as to why adversarial examples exist, including 
imperfections caused by the locally-linear nature of neural networks~\cite{ },  
%% [11] - Goodfellow, Ian J., Jonathon Shlens, and Christian Szegedy. "Explaining and harnessing adversarial examples." arXiv preprint arXiv:1412.6572 (2014).
``blind spots'' caused by non-ideal training or overfitting~\cite{ }, 
or that there is misalignment between the features used by humans and those learned by neural networks when performing the same classification task~\cite{ }.
% Adversarial Examples Are Not Bugs, They Are Features

\end{comment}
%
%%%%%%%

%Our attack instead aims to accurately synthesize forensic features used by a CNN, that are otherwise used to \textit{correctly} classify that image.  


%Instead of expoiting perturbations that cause a neural network to misclassify an image

By contrast,  our attack does not intend to exploit non-ideal properties of the classifier.  
Instead,  our attack aims to accurately synthesize the forensic features that a neural network would \textit{correctly} use to classify an unattacked image.
%Instead, our attack aims to accurately synthesize the forensic features that are used to \textit{correctly} classify an unattacked image. 
%
We are able to do this because forensic traces are typically not visible to the human eye.  
As a result, we can completely falsify these traces without modifying the contents of an image.  This approach may not translate well to attacks on classifiers for vision, because ideally the features learned by these classifier should correspond to visible attributes of an image.  
We believe that attempting to accurately synthesize `real' forensic features is the key to the transferability of our attack in zero-knowledge scenarios.  


Additionally,  adversarial example generation algorithms 
generally 
operate by creating perturbations
that are added to an image in order to fool a classifier.  
These perturbations 
are the same size as the input to the victim classifier.  
They are learned through an iterative process in which an intermediate version of the attacked image is presented to the victim classifier, gradient information is inferred, and the attack perturbation is updated.  As a result, a new perturbation must be iteratively learned for each image under attack.

By contrast our attack learns a convolutional generator which is trained in advance.   The generator is not modified or customized to the image under attack.   As a result, any image of arbitrary size can be passed through the generator, not just images with the same size as the victim CNN's input.  Additionally, our attack can be quickly deployed since it does not require iterative training for each new image.











%%%%%%%% WRITING NOTE %%%%%%%%
%From Carlini & Wagner, "Towards Evaluating the Robustness of Neural Networks"
%The key insight here is that by training to match the first network, we will hopefully avoid over-fitting against any of the training data. If the reason that neural networks exist is because neural networks are highly non-linear and have “blind spots” [46] where adversarial examples lie, then preventing this type of over-fitting might remove those blind spots.
%
% REFERENCE [46] - SZEGEDY, C., ZAREMBA, W., SUTSKEVER, I., BRUNA, J., ERHAN, D., GOODFELLOW, I., AND FERGUS, R. Intriguing properties of neural networks. ICLR (2013).
%
%
% IIn fact, as we will see later, defensive distillation does not remove adversarial examples. One potential reason this may occur is that others [11] have argued the reason adversarial examples exist is not due to blind spots in a highly non-linear neural network, but due only to the locally-linear nature of neural networks. This so-called linearity hypothesis appears to be true [47], and under this explanation it is perhaps less surprising that distillation does not increase the robustness of neural network
%
% [11] - Goodfellow, Ian J., Jonathon Shlens, and Christian Szegedy. "Explaining and harnessing adversarial examples." arXiv preprint arXiv:1412.6572 (2014).

% Adversarial Examples Are Not Bugs, They Are Features


==> sections/exp_setup.tex <==
%exp_setup
\section{Experimental Setup}
We conducted a series of experiments to demonstrate the effectiveness of the proposed attack in both white-box scenario and the zero-knowledge scenario.  In this section,  we talk about how we prepared the experimental datasets,  trained  victim forensic CNN detectors for evaluating the attacks,  and trained the proposed attacks.  %The following experiments were implemented using Tensorflow 1.14~\cite{tensorflow},  Nvidia GTX 1080,  GTX 1080Ti, and GTX 2080 GPUs.


\subsection{Datasets}
GANs have drawn attention recently, particularly since they can generate visually plausible human faces.  However, GANs are quite adept at generating a wide variety of objects.  To demonstrate the proposed attack is capable of falsifying forensic traces of GAN-generated images and fool forensic CNN detectors.  It is important to evaluate the proposed attack on both GAN-generated images of human faces and objects.  To do this,  we created two datasets,  one for images of human faces and the other for images of objects.  We now discuss how we prepared data for each dataset.  


\subhead{Human Face Dataset} This dataset consists of real images and GAN-generated images of human faces.   The GAN-generated images were created using StyleGAN~\cite{stylegankarras2019style},  StyleGAN2~\cite{stylegan2Karras2019},  and StarGAN-v2~\cite{starganv2choi2020}.  StyleGAN and StyleGAN2 generated images were downloaded from publicly available datasets shared by Nvidia Research Lab~\cite{stylegandatabase,  stylegan2database}. The StarGAN-v2 generated images were created using pre-trained StarGAN-v2 generator shared at~\cite{starganv2database}.   The real images were downloaded from FFHQ dataset~\cite{stylegan2Karras2019} and CelebA-HQ dataset~\cite{progankarras2017progressive}.  
In total,  the human face dataset contains $66,000$ real images with $44,000$ from FFHQ and $22,000$ from CelebA-HQ; $126,000$ GAN-generated images,  $42,000$ using StyleGAN,  $42,000$ using StyleGAN2,  and $42,000$ using StarGAN-v2. 

Next,  we partitioned the data into two disjoint training sets,   \textit{D-set} and \textit{A-set},  and an evaluation set,   \textit{Eval-set}.   \textit{D-set} was used to train the victim forensic CNN detectors.  It contains  $60,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2; and $60,000$ real images with $40,000$ from FFHQ and $20,000$ from CelebA-HQ.  \textit{A-set} was used to train the proposed attack.  Since training the proposed attack only requires GAN-generated images,  \textit{A-set} contains $60,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2.  

To demonstrate the effectiveness of the proposed attack,  we benchmarked the baseline performance of the victim forensic CNN detectors and evaluated the performance of our proposed attack against these CNNs using a common evaluation set, \textit{Eval-set}.  \textit{Eval-set} contains $6,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2; and $6,000$ real images with  $4,000$ from FFHQ and $2,000$ from CelebA-HQ. 
   
The resolutions of the StyleGAN and StyleGAN2 generated images,  and the real images of FFHQ and Celeb-A are all $1024\times 1024$.  The resolutions of the StarGAN-v2 generated images are $256\times 256$.

\subhead{Object Dataset}This dataset contains real images and GAN-generated images of objects.  The object dataset is a subset of publicly available ForenSynths dataset~\cite{wang2020cnn}.   The ForenSynths dataset was created to demonstrate that CNNs could learn general forensic traces of synthesized images.  Therefore CNNs trained on generated images produced by one GAN method can detect generated images produced by other generative models.  The training set of ForenSynths dataset contains only ProGAN generated images of objects and real images from LSUN dataset~\cite{yu2016lsun}. The testing set of ForenSynths dataset contains varying numbers of generated images produced by 12 different generative methods.  

From the training set of ForenSynths dataset,  we created two disjoint training sets,   \textit{D-set} for training victim CNN detectors and \textit{A-set} for training the proposed attack.  \textit{D-set} contains $50,000$ randomly selected ProGAN generated images and $50,000$ randomly selected real images.  Since training the proposed attack only requires GAN-generated images,  \textit{A-set} contains  $50,000$ randomly selected ProGAN generated images.  

To demonstrate the effectiveness of the proposed attack,  we benchmarked the baseline performance of victim forensic CNN detectors and evaluated the performance of our proposed attack against these CNNs using a common evaluation set,  \textit{Eval-set}.  \textit{Eval-set} contains $4,000$ real images from LSUN  and all the generated images of objects created by six different GAN methods from the testing set of ForenSynths dataset.   These GAN methods are ProGAN~\cite{progankarras2017progressive}, CycleGAN~\cite{cycleganzhu2017unpaired}, StyleGAN~\cite{stylegankarras2019style},  StyleGAN2~\cite{stylegan2Karras2019},  BigGAN~\cite{bigganbrock2018large},  and GauGAN~\cite{gauganpark2019gaugan}.  Since the numbers of images generated by each GAN method are different in the ForenSynths dataset,  we listed them in Table~\ref{tab: set1}.  
The resolution of  images in this dataset is $256\times 256$. 

The object dataset was created to demonstrate the proposed attack can be trained on images generated by one GAN method (ProGAN) and transfer to falsify forensic traces of images generated by other GAN methods (six other GAN methods in Table~\ref{tab: set1}) unseen by the attack. 

\begin{table}[!t]
\centering
\caption{The number of GAN-generated images  in the \textit{Eval-set} of the object dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccccc}
\textbf{GANs}& ProGAN&CycleGAN& StyleGAN& StyleGAN2& BigGAN& GauGAN\\
\hline
\textbf{No. of images} &4,000 & 1,300 &6,000 &8,000 &2,000 &5,000\\
\end{tabular}}
\label{tab: set1}
\end{table} 

\subsection{Victim Forensic CNN Detectors}
Before training and evaluating the proposed attack,  we  trained and benchmarked the performance of forensic CNNs on detecting GAN-generated images.  These forensic CNNs were trained as  binary classifiers  to differetiate between real images and GAN-generated images.  To fully evaluate the proposed attack,  in this paper we used eight state-of-the-art CNN models to train the CNN detectors.  These CNN models were designed for computer vision,  mulitmedia forensics,  or steganalysis.  They are  Xception~\cite{xception},  ResNet-50~\cite{resnet},  DenseNet~\cite{densenet},   MISLNet~\cite{mislnet},  PHNet~\cite{phnet},  SRNet~\cite{srnet},  Image CNN~\cite{transfernet},  and CamID CNN~\cite{tuama}.   We trained each forensic CNN individually using \textit{D-set} of the human face dataset and the object dataset.  It yielded 16 CNN detectors in total and formed the set of victim forensic CNN detectors we attacked in this paper.  

All CNN detectors were trained from scratch for 20 epochs on both datasets.   The predictions were made from $256\times 256$ image patches.  For images of resolution $1024\times 1024$,  we randomly cropped a $256\times 256$ image patch from each full-size image during training and testing the CNN detectors.  We chose the best set of hyperparameters for each CNN detector that yields the highest classification accuracy after grid search.  For Xception the learning rate started at $0.01$;  for ResNet-50 the learning rate started at $0.0001$ and for all other CNNs the learning rate started at $0.0005$.  These learning rates decayed by half every 4 epochs.  Weights were initialized using Xavier initializer~\cite{xavier} and biases were initialized as $0$'s.  Weights and biases were optimized using stochastic gradient descent. 


To benchmark the performance of the victim CNN detectors,  we calculated the classification accuracy achieved by each CNN detector. The classification accuracy is defined as the percentage of the real and GAN-generated images that were correctly classified by the CNN detector out of  all images in \textit{Eval-set}.   

\begin{comment}
\begin{equation}
Acc.=\frac{Number of correctly classified real + number  of correctly classified generated}{Total number of testing data}
\end{equation}
\end{comment}

The classification accuracy achieved by each victim CNN detector on  both datasets are shown in Table~\ref{tab: acc}.  On average,  we achieved $95.94\%$ classification accuracy on the human face dataset and $99.14\%$ classification accuracy on the object dataset.   The results showed that the CNN detectors used  in this paper were not biased.  . 
 
Additionally,  since the goal of this paper is to attack GAN-generated images and  fool CNN detectors,  we wanted to compare the performance of the victim CNN detectors on classifying GAN-generated images before and after the attack being launched.   To do this,  we calculated the recalls of classifying GAN-generated images.  The recall associated with one particular pair of CNN detector and GAN method is defined as the percentage of the GAN-generated images that were correctly detected by the CNN detector out of the generated images produced by that GAN method. 

Table~\ref{tab: recall_face} shows the recalls achieved by each victim CNN detector on the  human face dataset.  Each entry is associated with one victim CNN detector and  one  GAN method.  The average recall achieved on the human face dataset is  $ 94.53\%$.   The recall on classifying StarGAN-v2 generated image is $98.66\%$,  on classifying StyleGAN generated images is $92.15\%$,  and on classifying StyleGAN2 generated image is $92.77\%$.  The results showed that the CNN detectors can reliably detect GAN-generated images of human faces before the attack being launched. 

Table~\ref{tab: recall_object} shows the recalls  achieved by each victim CNN detector on the object dataset.  Each entry is associated with one victim CNN detector and  one  GAN method.  The average recall achieved on the object dataset is   $77.12\%$.  The results are consistent with previous research by Wang et al. ~\cite{wang2020cnn},  and showed that the CNN detectors can reliably detect GAN-generated images of objects  before the attack being launched. 

The baseline performance of the victim forensic CNN detectors demonstrated  that  CNN detectors used in this paper were well-trained,  and can be used  to evaluate the proposed attack in the following experiments. 

\begin{table}[!t]
\centering
\caption{Baseline classification accuracies of the victim CNN detectors achieved on the human face dataset and  the object dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c||c}
\hline
\textbf{CNNs} &\textbf{ Human Face Dataset}&  \textbf{Object Dataset}\\
\hline
\textbf{Xception} &99.67\%&99.75\% \\
\textbf{ResNet-50}& 78.26\%&99.14\%\\
\textbf{DenseNet} &96.39\%&97.04\%\\
\textbf{MISLNet}& 99.93\%&99.15\%\\
\textbf{PHNet} & 95.15\%&99.73\%\\
\textbf{SRNet} &99.50\% &99.78\%\\
\textbf{Image CNN}& 99.49\% & 99.10\%\\
\textbf{CamID CNN} & 99.16\%& 99.46\%\\
\textbf{Avg.}&\textbf{95.94\%} & textbf{99.14\%}\\
\hline
\end{tabular}}
\label{tab: acc}
\end{table}

\begin{table}[!t]
\centering
\caption{Recalls of detecting GAN-generated images of human faces by the victim forensic CNN detectors. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{CNNs} & \textbf{StarGAN-v2} &\textbf{StyleGAN} &\textbf{StyleGAN2}&\textcolor{blue}{\textbf{Avg.}}\\
\hline
\textbf{Xception}&99.92\% & 99.90\%&100.00\% &99.94\%\\
\textbf{ResNet-50}&95.65\% & 49.12\% & 67.62\%&70.80\%\\
\textbf{DenseNet} &98.40\%&96.27\% &99.22\% &97.96\%\\
\textbf{MISLNet}&99.95\%  &99.97\% &100.00\%&99.97\%\\
\textbf{PHNet} & 97.37\% & 93.65\% &76.00\%&89.01\%\\
\textbf{SRNet}  & 99.27\%& 99.75\% &99.80\%&99.61\%\\
\textbf{Image CNN}& 99.95\% &99.12\% &99.90\%&99.66\%  \\
\textbf{CamID CNN} &98.77\% &99.42\% & 99.65\%&99.28\%\\
\textcolor{blue}{\textbf{Avg.}}& \textcolor{blue}{\textbf{98.66\%}}& \textcolor{blue}{\textbf{92.15\%}}&\textcolor{blue}{\textbf{92.77\%}}&\textcolor{blue}{\textbf{94.53\%}}\\
\hline
\end{tabular}}
\label{tab: recall_face}
\end{table}


\begin{table} [!t]
\centering
\caption{Recalls of detecting GAN-generated images of objects by the victim forensic CNN detectors.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg. }\\
\hline
\textbf{Xception}&99.82\%&69.56\% &70.92\% & 72.91\% &19.61\%& 34.50\%&\textbf{61.22\%}\\
\textbf{ResNet-50} &99.65\%& 77.08\% &77.06\% & 92.41\% &82.40\% &82.29\%&\textbf{85.15\%}  \\
\textbf{DenseNet}&96.90\% & 77.70\%&61.98\% &88.69\% &78.75\% & 80.93\%&\textbf{80.83\%}\\
\textbf{MISLNet}&98.80\% & 73.16\%& 89.59\%&78.14\% & 73.05\% & 34.45\%&\textbf{74.53\%} \\
\textbf{PHNet} &99.78\% &65.34\% &76.34\%& 89.61\%&79.80\%&57.49\%&\textbf{78.06\%}\\
\textbf{SRNet} &99.72\%& 100.00\% &69.68\% & 33.50\%& 99.85\%&99.76\%&\textbf{ 83.75\%}\\
\textbf{Image CNN}&99.90\% &41.89\% & 92.97\%& 97.40\% &86.35\% &80.40\%&\textbf{83.15\%}\\
\textbf{CamID CNN} & 99.70\%& 43.54\% & 71.37\% & 79.53\% & 68.25\%&59.31\%&\textbf{70.28\%} \\
\textbf{Avg.}&\textbf{99.28\%}&\textbf{68.53\%}&\textbf{76.24\%}&\textbf{79.02\%}&\textbf{73.51\%}&\textbf{66.14\%}&\textbf{77.12\%}\\
\hline
\end{tabular}}
\label{tab: recall_object}
\end{table}


\subsection{Attack Evaluation Metrics}
A successful anti-forensic attack should be able to fool forensic CNN detectors with high probability,  and maintain high visual quality.   We used the following metrics  to evaluate the  proposed  attack on fooling the CNN detectors and the visual quality of the attacked images. 

\subhead{Attack Success Rate} To evaluate the performance of the proposed attack in terms of  fooling  the victim CNN detectors,  we define the  attack success rate  as the percentage of the attacked images that are classified as ``real" by the victim CNN detector.

\subhead{Image Quality} To  evaluate the visual quality of  attacked images produced by the proposed attack,  we calculated the mean PSNR and mean SSIM between the  GAN-generated images and the attacked images. 


\subsection{White-Box Attack}
The first set of experiments is to demonstrate the effectiveness of proposed attack in the white-box scenario.  In the white-box scenario,  we assume the attacker has access to the victim CNN detector.   Therefore,  the attacker can train an anti-forensic generator directly against the victim  CNN detector he/she is attempting to fool. 

For  each victim  CNN detector  trained on the  human face dataset and the object dataset,   we trained an individual anti-forensic generator to attack it.  To evaluate the performance of each trained anti-forensic generator,  we used the generator to attack each GAN-generated image in the \textit{Eval-set},   saving the attacked images to  disk as PNG files.   This is to ensure the pixel values of  attacked images reside in the range from 0 to 255.   Next,  we calculated the attack success rate  by using the victim CNN detector  to classify the attacked images.  We also calculated the mean PSNR and mean SSIM between the GAN-generated images and the attacked images to evaluate the visual quality of the attacked images.  

The anti-forensic generators presented in this paper were trained from scratch for 32 epochs.  Learning rate was $0.0001$.  Weights were initialized using Xavier initializer~\cite{xavier} and biases were initialized as $0$'s.  Weights and biases were optimized using stochastic gradient descent.   To balance the image  quality and attack success rates,  $\alpha$ in equation~\ref{eq:g_loss} was chosen after a grid search range from $1$ to $200$ with an increment of $20$.  Specifically,  $\alpha$ was chosen to be $20$ when attacking the victim CNN detectors trained  on the  human face dataset and $\alpha$ was chosen to be $100$ when  attacking victim CNN detectors trained on the object dataset.  For images of resolution $1024\times 1024$  in the   human face  dataset,  we randomly cropped $256\times 256$ image patches  for training the proposed attack.

\subhead{Comparing with Other Generators}Additionally,  we compared the performance of the proposed anti-forensic generator with two other generators used in  previous GAN-based attacks.  Kim et al.  used a residual generator adversarially trained to remove median filtering traces~\cite{residualgan}.  Chen et al.  used MISLGAN generator trained to  falsify forensic traces of camera models.   We repeated experiments on both datasets using the residual generator and the MISLGAN generator.   We note that to improve the visual quality of images produced by the comparing generators,   $\alpha$ was chosen to be $200$ (much higher than the proposed generator).  

\subsection{Zero Knowledge Attack}
This set of experiments was conducted to evaluate the proposed attack In the zero knowledge scenario.  We assume the attacker has no knowledge about the victim CNN detector that the investigator would use to classify images.  Particularly,  the attacker has no access to the victim CNN detector and cannot observe any input or output of the CNN detector,  since the investigator may use a private CNN detector that the attacker by all means cannot have access to.   This is a more realistic yet challenging scenario. 
In the zero-knowledge scenario,   we evaluated the transferability of the proposed attack to attack unseen CNN detectors.  

To achieve the transferability,  we built an ensemble of forensic CNN detectors to train the proposed anti-forensic generator.   To mimic the zero knowledge scenario,   each ensemble used to train the proposed attack did not include the CNN detector used for evaluating the attack.    We assume that if the attacker has no knowledge of the  CNN detector,  the attacker may use all available CNN detectors to make the attack as strong as possible.    However,  due to the limitation of computer memory,  the Xception was always excluded from the ensemble when attacking other networks. 

We used the same hyperparameters and $\alpha$  as in the white-box scenario to train proposed attack. 





==> sections/exp_setup_v1.tex <==
%exp_setup

\section{Experimental Setup}
%We conducted a series of experiments to demonstrate the effectiveness of the proposed attack in both white-box scenario and the zero-knowledge scenario.  In this section,  we talk about how we prepared the experimental datasets,  trained  victim forensic CNN detectors for evaluating the attacks,  and trained the proposed attacks.  

In this section, we provide details of the experimental evaluation of our proposed attack, including the  datasets used in our experiments, the baseline performance of the forensic CNNs we attacked, and the procedure used to evaluate our white-box and zero-knowledge attack.


\subsection{Datasets}
%GANs have drawn attention recently, particularly since they can generate visually plausible human faces.  However, GANs are quite adept at generating a wide variety of objects.  To demonstrate the proposed attack is capable of falsifying forensic traces of GAN-generated images and fool forensic CNN detectors.  It is important to evaluate the proposed attack on both GAN-generated images of human faces and objects.  To do this,  we created two datasets,  one for images of human faces and the other for images of objects.  We now discuss how we prepared data for each dataset.  

We created two datasets to evaluate our attacks, each containing both real and GAN-generated images.  The first dataset contains only images of human faces, while the second contains images of non-human objects. 



\subhead{Human Face Dataset} This dataset consists of real images and GAN-generated images of human faces.   The GAN-generated images were created using StyleGAN~\cite{stylegankarras2019style},  StyleGAN2~\cite{stylegan2Karras2019},  and StarGAN-v2~\cite{starganv2choi2020}.  StyleGAN and StyleGAN2 generated images were downloaded from publicly available datasets shared by Nvidia Research Lab~\cite{stylegandatabase,  stylegan2database}. The StarGAN-v2 generated images were created using pre-trained StarGAN-v2 generator shared at~\cite{starganv2database}.   The real images were downloaded from FFHQ dataset~\cite{stylegan2Karras2019} and CelebA-HQ dataset~\cite{progankarras2017progressive}.  
In total,  the human face dataset contains $66,000$ real images with $44,000$ from FFHQ and $22,000$ from CelebA-HQ; $126,000$ GAN-generated images,  $42,000$ using StyleGAN,  $42,000$ using StyleGAN2,  and $42,000$ using StarGAN-v2.  
 %
The size of all StyleGAN and StyleGAN2 generated images,  as well as the real images from the FFHQ and Celeb-A are all $1024\times 1024$ pixels.  The size of StarGAN-v2 generated images are $256\times 256$.

Next,  we partitioned the data into two disjoint training sets, the  \textit{D-set} and the \textit{A-set},  as well as an evaluation set  \textit{Eval-set}.   The \textit{D-set} was used to train the victim forensic CNN detectors.  It contains  $60,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2; and $60,000$ real images with $40,000$ from FFHQ and $20,000$ from CelebA-HQ.  The \textit{A-set} was used to train the proposed attack.  Since training the proposed attack only requires GAN-generated images,  \textit{A-set} contains $60,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2.  




To demonstrate the effectiveness of the proposed attack,  we benchmarked the baseline performance of the victim forensic CNN detectors and evaluated the performance of our proposed attack against these CNNs using a common evaluation set, \textit{Eval-set}.  The \textit{Eval-set} contains $6,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2; and $6,000$ real images with  $4,000$ from FFHQ and $2,000$ from CelebA-HQ. 
   
%The resolutions of the StyleGAN and StyleGAN2 generated images,  and the real images of FFHQ and Celeb-A are all $1024\times 1024$.  The resolutions of the StarGAN-v2 generated images are $256\times 256$.

\subhead{Object Dataset}This dataset contains real images and GAN-generated images of objects.  The object dataset is a subset of publicly available ForenSynths dataset~\cite{wang2020cnn}.   The ForenSynths dataset was created to demonstrate that CNNs could learn general forensic traces of synthesized images.  Therefore CNNs trained on generated images produced by one GAN method can detect generated images produced by other generative models.  The training set of ForenSynths dataset contains only ProGAN generated images of objects and real images from LSUN dataset~\cite{yu2016lsun}. The testing set of ForenSynths dataset contains varying numbers of generated images produced by 12 different generative methods.  

From the training set of the ForenSynths dataset,  we created two disjoint training sets:   \textit{D-set} for training victim CNN detectors and \textit{A-set} for training the proposed attack.  \textit{D-set} contains $50,000$ randomly selected ProGAN generated images and $50,000$ randomly selected real images.  Since training the proposed attack only requires GAN-generated images,  \textit{A-set} contains  $50,000$ randomly selected ProGAN generated images.  

To demonstrate the effectiveness of the proposed attack,  we benchmarked the baseline performance of victim forensic CNN detectors and evaluated the performance of our proposed attack against these CNNs using a common evaluation set,  \textit{Eval-set}.  \textit{Eval-set} contains $4,000$ real images from LSUN  and all the generated images of objects created by six different GAN methods from the testing set of ForenSynths dataset.   These GAN methods are ProGAN~\cite{progankarras2017progressive}, CycleGAN~\cite{cycleganzhu2017unpaired}, StyleGAN~\cite{stylegankarras2019style},  StyleGAN2~\cite{stylegan2Karras2019},  BigGAN~\cite{bigganbrock2018large},  and GauGAN~\cite{gauganpark2019gaugan}.  Since the numbers of images generated by each GAN method are different in the ForenSynths dataset,  we listed them in Table~\ref{tab: set1}.  
%The resolution of  images in this dataset is $256\times 256$. 
%
The object dataset was created to demonstrate the proposed attack can be trained on images generated by one GAN method (ProGAN) and transfer to falsify forensic traces of images generated by other GAN methods (six other GAN methods in Table~\ref{tab: set1}) unseen by the attack. 


\subsection{Victim Forensic CNN Detectors}
Before training and evaluating the proposed attack,  we  trained and benchmarked the performance of forensic CNNs on detecting GAN-generated images.  These forensic CNNs were trained as  binary classifiers  to differetiate between real images and GAN-generated images.  To  evaluate our proposed attack,  we used eight state-of-the-art CNN models %to train the CNN detectors.  
trained as {\gi} detectors.  
These CNN models were designed for computer vision,  mulitmedia forensics,  or steganalysis.  They are  Xception~\cite{xception},  ResNet-50~\cite{resnet},  DenseNet~\cite{densenet},   MISLNet~\cite{mislnet},  PHNet~\cite{phnet},  SRNet~\cite{srnet},  Image CNN~\cite{transfernet},  and CamID CNN~\cite{tuama}.   We trained each forensic CNN individually using \textit{D-set} of the human face dataset and the object dataset.  This yielded 16 CNN detectors in total and formed the set of victim %forensic CNN detectors 
classifiers we attacked in this paper.  

\begin{table}[!t]
\centering
\caption{The number of GAN-generated images  in the \textit{Eval-set} of the object dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccccc}
\textbf{GANs}& ProGAN&CycleGAN& StyleGAN& StyleGAN2& BigGAN& GauGAN\\
\hline
\textbf{No. of images} &4,000 & 1,300 &6,000 &8,000 &2,000 &5,000\\
\end{tabular}}
\label{tab: set1}
\end{table} 
%\vspace{2em}

%%
All CNN detectors were trained from scratch for 20 epochs on both datasets.   
%
%Predictions were made from $256\times 256$ image patches.  
The input size of each CNN was a $256\times 256$ image.  
For images of resolution $1024\times 1024$,  we randomly cropped a $256\times 256$ pixel patch from each image during training and testing. % the detectors.
%
%%  
We chose the set of hyperparameters for each CNN  that yielded the highest classification accuracy after a grid search.  For Xception the learning rate started at $0.01$;  for ResNet-50 the learning rate started at $0.0001$ and for all other CNNs the learning rate started at $0.0005$.  These learning rates decayed by half every 4 epochs.  Weights were initialized using Xavier initializer~\cite{xavier}, biases were initialized as $0$'s, and both were optimized using stochastic gradient descent.  

%Weights and biases were optimized using stochastic gradient descent. 


To benchmark the performance of the victim CNN detectors,  we calculated the classification accuracy achieved by each CNN detector. The classification accuracy is defined as the percentage of the real and GAN-generated images that were correctly classified by the CNN detector out of  all images in \textit{Eval-set}.   
%
%
The classification accuracy achieved by each victim CNN detector on  both datasets are shown in Table~\ref{tab: acc}.  On average,  we achieved $95.94\%$ classification accuracy on the human face dataset and $99.14\%$ classification accuracy on the object dataset.   The results showed that the CNN detectors used  in this paper were not biased.  

\begin{table}[!t]
\centering
\caption{Baseline classification accuracies of the victim CNN detectors achieved on the human face dataset and  the object dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c||c}
\hline
\textbf{CNNs} &\textbf{ Human Face Dataset}&  \textbf{Object Dataset}\\
\hline
\textbf{Xception} &99.67\%&99.75\% \\
\textbf{ResNet-50}& 78.26\%&99.14\%\\
\textbf{DenseNet} &96.39\%&97.04\%\\
\textbf{MISLNet}& 99.93\%&99.15\%\\
\textbf{PHNet} & 95.15\%&99.73\%\\
\textbf{SRNet} &99.50\% &99.78\%\\
\textbf{Image CNN}& 99.49\% & 99.10\%\\
\textbf{CamID CNN} & 99.16\%& 99.46\%\\
\textbf{Avg.}&\textbf{95.94\%} & \textbf{99.14\%}\\
\hline
\end{tabular}}
\label{tab: acc}
\end{table}
 
 \begin{comment}
Additionally,  since the goal of this paper is to attack GAN-generated images and  fool CNN detectors,  we wanted to compare the performance of the victim CNN detectors on classifying GAN-generated images before and after the attack being launched.   To do this,  we calculated the recalls of classifying GAN-generated images.  The recall associated with one particular pair of CNN detector and GAN method is defined as the percentage of the GAN-generated images that were correctly detected by the CNN detector out of the generated images produced by that GAN method. 

Table~\ref{tab: recall_face} shows the recalls achieved by each victim CNN detector on the  human face dataset.  Each entry is associated with one victim CNN detector and  one  GAN method.  The average recall achieved on the human face dataset is  $ 94.53\%$.   The recall on classifying StarGAN-v2 generated image is $98.66\%$,  on classifying StyleGAN generated images is $92.15\%$,  and on classifying StyleGAN2 generated image is $92.77\%$.  The results showed that the CNN detectors can reliably detect GAN-generated images of human faces before the attack being launched. 

Table~\ref{tab: recall_object} shows the recalls  achieved by each victim CNN detector on the object dataset.  Each entry is associated with one victim CNN detector and  one  GAN method.  The average recall achieved on the object dataset is   $77.12\%$.  The results are consistent with previous research by Wang et al. ~\cite{wang2020cnn},  and showed that the CNN detectors can reliably detect GAN-generated images of objects  before the attack being launched. 

The baseline performance of the victim forensic CNN detectors demonstrated  that  CNN detectors used in this paper were well-trained,  and can be used  to evaluate the proposed attack in the following experiments. 



\begin{table}[!t]
\centering
\caption{Recalls of detecting GAN-generated images of human faces by the victim forensic CNN detectors. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{CNNs} & \textbf{StarGAN-v2} &\textbf{StyleGAN} &\textbf{StyleGAN2}&\textcolor{blue}{\textbf{Avg.}}\\
\hline
\textbf{Xception}&99.92\% & 99.90\%&100.00\% &99.94\%\\
\textbf{ResNet-50}&95.65\% & 49.12\% & 67.62\%&70.80\%\\
\textbf{DenseNet} &98.40\%&96.27\% &99.22\% &97.96\%\\
\textbf{MISLNet}&99.95\%  &99.97\% &100.00\%&99.97\%\\
\textbf{PHNet} & 97.37\% & 93.65\% &76.00\%&89.01\%\\
\textbf{SRNet}  & 99.27\%& 99.75\% &99.80\%&99.61\%\\
\textbf{Image CNN}& 99.95\% &99.12\% &99.90\%&99.66\%  \\
\textbf{CamID CNN} &98.77\% &99.42\% & 99.65\%&99.28\%\\
\textcolor{blue}{\textbf{Avg.}}& \textcolor{blue}{\textbf{98.66\%}}& \textcolor{blue}{\textbf{92.15\%}}&\textcolor{blue}{\textbf{92.77\%}}&\textcolor{blue}{\textbf{94.53\%}}\\
\hline
\end{tabular}}
\label{tab: recall_face}
\end{table}


\begin{table} [!t]
\centering
\caption{Recalls of detecting GAN-generated images of objects by the victim forensic CNN detectors.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textcolor{blue}{\textbf{Avg. }}\\
\hline
\textbf{Xception}&99.82\%&69.56\% &70.92\% & 72.91\% &19.61\%& 34.50\%&61.22\%\\
\textbf{ResNet-50} &99.65\%& 77.08\% &77.06\% & 92.41\% &82.40\% &82.29\%&85.15\%  \\
\textbf{DenseNet}&96.90\% & 77.70\%&61.98\% &88.69\% &78.75\% & 80.93\%&80.83\%\\
\textbf{MISLNet}&98.80\% & 73.16\%& 89.59\%&78.14\% & 73.05\% & 34.45\%&74.53\% \\
\textbf{PHNet} &99.78\% &65.34\% &76.34\%& 89.61\%&79.80\%&57.49\%&78.06\%\\
\textbf{SRNet} &99.72\%& 100.00\% &69.68\% & 33.50\%& 99.85\%&99.76\%& 83.75\%\\
\textbf{Image CNN}&99.90\% &41.89\% & 92.97\%& 97.40\% &86.35\% &80.40\%&83.15\%\\
\textbf{CamID CNN} & 99.70\%& 43.54\% & 71.37\% & 79.53\% & 68.25\%&59.31\%&70.28\% \\
\textcolor{blue}{\textbf{Avg.}} &\textcolor{blue}{\textbf{99.28\%}}&\textcolor{blue}{\textbf{68.53\%}}&\textcolor{blue}{\textbf{76.24\%}}&\textcolor{blue}{\textbf{79.02\%}}&\textcolor{blue}{\textbf{73.51\%}}&\textcolor{blue}{\textbf{66.14\%}}&\textcolor{blue}{\textbf{77.12\%}}\\
\hline
\end{tabular}}
\label{tab: recall_object}
\end{table}
\end{comment}

%\subsection{Attack Evaluation Metrics}
%A successful anti-forensic attack should be able to fool forensic CNN detectors with high probability,  and maintain high visual quality.   We used the following metrics  to evaluate the  proposed  attack on fooling the CNN detectors and the visual quality of the attacked images. 

%\subhead{Attack Success Rate} To evaluate the performance of the proposed attack in terms of  fooling  the victim CNN detectors,  we define the  attack success rate  as the percentage of the attacked images that are classified as ``real" by the victim CNN detector.

%\subhead{Image Quality} To  evaluate the visual quality of  attacked images produced by the proposed attack,  we calculated the mean PSNR and mean SSIM between the  GAN-generated images and the attacked images. 


\subsection{White-Box Attack}
The first set of experiments was designed to evaluate the effectiveness of our proposed attack in the white-box scenario.  Here, we assume the attacker has access to the victim classifier and can train  directly against it.

%In the white-box scenario,  we assume the attacker has access to the victim CNN detector.   Therefore,  the attacker can train an anti-forensic generator directly against the victim  CNN detector he/she is attempting to fool. 

For  each victim CNN detector trained on the  human face dataset and the object dataset,   we trained an individual anti-forensic generator to attack it.  To evaluate the performance of the anti-forensic generator,  we used the generator to attack each GAN-generated image in the \textit{Eval-set},   saving the attacked images to  disk as PNG files.   This is to ensure the pixel values of  attacked images reside in the range from 0 to 255.   Next,  we calculated the attack success rate  by using the victim CNN detector  to classify the attacked images.  We also calculated the mean PSNR and mean SSIM between the GAN-generated images and the attacked images to evaluate the visual quality of the attacked images.  

%%%
The anti-forensic generators presented in this paper were trained from scratch for 32 epochs with a learning rate of $0.0001$.  
Weights were initialized using Xavier initializer~\cite{xavier} and biases were initialized as $0$'s, and were optimized using stochastic gradient descent. 
%Weights and biases were optimized using stochastic gradient descent.   
%
To balance the image  quality and attack success rates,  $\alpha$ in equation~\ref{eq:g_loss} was chosen after a grid search range from $1$ to $200$ with an increment of $20$.  Specifically,  $\alpha$ was chosen to be $20$ 
for attacks on the human face dataset and $100$ for attacks on the object dataset. 
%when attacking the victim CNN detectors trained  on the  human face dataset and $\alpha$ was chosen to be $100$ when  attacking victim CNN detectors trained on the object dataset.  
When training our attack on the human face dataset, we randomly cropped $256\times 256$  patches from images of size $1024\times 1024$ .
%For images of resolution $1024\times 1024$  in the   human face  dataset,  we randomly cropped $256\times 256$ image patches  for training the proposed attack.


%For images of resolution $1024\times 1024$  in the   human face  dataset,  we randomly cropped $256\times 256$ image patches  for training the proposed attack.

\subhead{Comparing with Other Generators} We compared the performance of the proposed anti-forensic generator with two other generators used in  previous GAN-based attacks.  Kim et al.  used a residual generator adversarially trained to remove median filtering traces~\cite{residualgan}.  Chen et al.  used MISLGAN generator trained to  falsify forensic traces of camera models.   We repeated experiments on both datasets using the residual generator and the MISLGAN generator.   
%We note that to improve the visual quality of images produced by the comparing generators,   $\alpha$ was chosen to be $200$ (much higher than the proposed generator).  

\subsection{Zero-Knowledge Attack}
This set of experiments was conducted to evaluate the proposed attack in the zero-knowledge scenario.  We assume the attacker has no knowledge about the victim CNN detector that the investigator would use to classify images.  Particularly,  the attacker has no access to the victim CNN detector and cannot observe any input or output of the CNN detector,  since the investigator may use a private CNN detector that the attacker by all means cannot have access to.   This is a more realistic yet challenging scenario. 
In the zero-knowledge scenario,   we evaluated the transferability of the proposed attack to attack unseen CNN detectors.  

To achieve the transferability,  we built an ensemble of forensic CNN detectors to train the proposed anti-forensic generator.   To mimic the zero-knowledge scenario,   each ensemble used to train the %proposed
attack did not include 
%the CNN detector used for evaluating the attack.
the victim classifier.  
 We assume that if the attacker has no knowledge of the % CNN detector
 victim classifier's architecture,  
%the attacker will use all available CNN detectors to make the attack as strong as possible.    
the attacker will use  all available CNNs in their ensemble to strenthen their attack.   
%However,  due to the limitation of computer memory,  the Xception was always excluded from the ensemble when attacking other networks.  
However, due to limited GPU memory, Xception was always excluded from the training ensemble in our experiments. 
During training, we used the same hyperparameters and other settings as the white-box scenario. 


%We used the same hyperparameters and $\alpha$  as in the white-box scenario to train proposed attack. 





==> sections/exp_setup_v2_icpr.tex <==
%exp_setup

\section{Experimental Setup}
%We conducted a series of experiments to demonstrate the effectiveness of the proposed attack in both white-box scenario and the zero-knowledge scenario.  In this section,  we talk about how we prepared the experimental datasets,  trained  victim forensic CNN detectors for evaluating the attacks,  and trained the proposed attacks.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%   Below Removed To Save Space    %
%                                                     %
\begin{comment}

In this section, we provide details of the experimental evaluation of our proposed attack, including the  datasets used in our experiments, the baseline performance of the forensic CNNs we attacked, and the procedure used to evaluate our white-box and zero-knowledge attack.

\end{comment}
%                                                     %
%   Above Removed To Save Space   %
%                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Datasets}
%GANs have drawn attention recently, particularly since they can generate visually plausible human faces.  However, GANs are quite adept at generating a wide variety of objects.  To demonstrate the proposed attack is capable of falsifying forensic traces of GAN-generated images and fool forensic CNN detectors.  It is important to evaluate the proposed attack on both GAN-generated images of human faces and objects.  To do this,  we created two datasets,  one for images of human faces and the other for images of objects.  We now discuss how we prepared data for each dataset.  

We created two datasets to evaluate our attacks, each containing both real and GAN-generated images.  The first dataset contains only images of human faces, while the second contains images of non-human objects. 



\subhead{Human Face Dataset} This dataset consists of real images and GAN-generated images of human faces.   The GAN-generated images were created using StyleGAN~\cite{stylegankarras2019style},  StyleGAN2~\cite{stylegan2Karras2019},  and StarGAN-v2~\cite{starganv2choi2020}.  StyleGAN and StyleGAN2 generated images were downloaded from publicly available datasets shared by Nvidia Research Lab~\cite{stylegandatabase,  stylegan2database}. The StarGAN-v2 generated images were created using pre-trained StarGAN-v2 generator shared at~\cite{starganv2database}.   The real images were downloaded from FFHQ dataset~\cite{stylegan2Karras2019} and CelebA-HQ dataset~\cite{progankarras2017progressive}.  
In total,  the human face dataset contains $66,000$ real images with $44,000$ from FFHQ and $22,000$ from CelebA-HQ; $126,000$ GAN-generated images,  $42,000$ using StyleGAN,  $42,000$ using StyleGAN2,  and $42,000$ using StarGAN-v2.  
 %
The size of all StyleGAN and StyleGAN2 generated images,  as well as the real images from the FFHQ and Celeb-A are all $1024\times 1024$ pixels.  The size of StarGAN-v2 generated images are $256\times 256$.

Next,  we partitioned the data into two disjoint training sets, the  \textit{D-set} and the \textit{A-set},  as well as an evaluation set  \textit{Eval-set}.   The \textit{D-set} was used to train the victim forensic CNN detectors.  It contains  $60,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2; and $60,000$ real images with $40,000$ from FFHQ and $20,000$ from CelebA-HQ.  The \textit{A-set} was used to train the proposed attack.  Since training the proposed attack only requires GAN-generated images,  \textit{A-set} contains $60,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2.  


To demonstrate the effectiveness of the proposed attack,  we benchmarked the baseline performance of the victim forensic CNN detectors and evaluated the performance of our proposed attack against these CNNs using a common evaluation set, \textit{Eval-set}.  The \textit{Eval-set} contains $6,000$ GAN-generated images drawn equally from StyleGAN,  StyleGAN2 and StarGAN-v2; and $6,000$ real images with  $4,000$ from FFHQ and $2,000$ from CelebA-HQ. 
   
%The resolutions of the StyleGAN and StyleGAN2 generated images,  and the real images of FFHQ and Celeb-A are all $1024\times 1024$.  The resolutions of the StarGAN-v2 generated images are $256\times 256$.

\subhead{Object Dataset}This dataset contains real images and GAN-generated images of objects.  The object dataset is a subset of publicly available ForenSynths dataset~\cite{wang2020cnn}.   The ForenSynths dataset was created to demonstrate that CNNs could learn general forensic traces of synthesized images.  Therefore CNNs trained on generated images produced by one GAN method can detect generated images produced by other generative models.  The training set of ForenSynths dataset contains only ProGAN generated images of objects and real images from LSUN dataset~\cite{yu2016lsun}. The testing set of ForenSynths dataset contains varying numbers of generated images produced by 12 different generative methods.  

From the training set of the ForenSynths dataset,  we created two disjoint training sets:   \textit{D-set} for training victim CNN detectors and \textit{A-set} for training the proposed attack.  \textit{D-set} contains $50,000$ randomly selected ProGAN generated images and $50,000$ randomly selected real images.  Since training the proposed attack only requires GAN-generated images,  \textit{A-set} contains  $50,000$ randomly selected ProGAN generated images.  

To demonstrate the effectiveness of the proposed attack,  we benchmarked the baseline performance of victim forensic CNN detectors and evaluated the performance of our proposed attack against these CNNs using a common evaluation set,  \textit{Eval-set}.  \textit{Eval-set} contains $4,000$ real images from LSUN  and all the generated images of objects created by six different GAN methods from the testing set of ForenSynths dataset.   
%
The ForenSynth dataset consists of 26,300 images comprised of 4,000 images from ProGAN~\cite{progankarras2017progressive}, 1,300 from CycleGAN~\cite{cycleganzhu2017unpaired}, 6,000 from StyleGAN~\cite{stylegankarras2019style},  8,000 from StyleGAN2~\cite{stylegan2Karras2019},  2,000 from BigGAN~\cite{bigganbrock2018large},  and 5,000 from GauGAN~\cite{gauganpark2019gaugan}.


%4,000+1,300 + 6,000 + 8,000+2,000+5,000

%These GAN methods are ProGAN~\cite{progankarras2017progressive}, CycleGAN~\cite{cycleganzhu2017unpaired}, StyleGAN~\cite{stylegankarras2019style},  StyleGAN2~\cite{stylegan2Karras2019},  BigGAN~\cite{bigganbrock2018large},  and GauGAN~\cite{gauganpark2019gaugan}.  Since the numbers of images generated by each GAN method are different in the ForenSynths dataset,  we listed them in Table~\ref{tab: set1}.  






%The resolution of  images in this dataset is $256\times 256$. 
%
%The object dataset was created to demonstrate the proposed attack can be trained on images generated by one GAN method (ProGAN) and transfer to falsify forensic traces of images generated by other GAN methods (six other GAN methods in Table~\ref{tab: set1}) unseen by the attack. 


\subsection{Victim Forensic CNN Detectors}
Before training and evaluating the proposed attack,  we  trained and benchmarked the performance of forensic CNNs on detecting GAN-generated images.  These forensic CNNs were trained as  binary classifiers  to differetiate between real images and GAN-generated images.  To  evaluate our proposed attack,  we used eight state-of-the-art CNN models %to train the CNN detectors.  
trained as {\gi} detectors.  
These CNN models were designed for computer vision,  mulitmedia forensics,  or steganalysis.  They are  Xception~\cite{xception},  ResNet-50~\cite{resnet},  DenseNet~\cite{densenet},   MISLNet~\cite{mislnet},  PHNet~\cite{phnet},  SRNet~\cite{srnet},  Image CNN~\cite{transfernet},  and CamID CNN~\cite{tuama}.   We trained each forensic CNN individually using \textit{D-set} of the human face dataset and the object dataset.  This yielded 16 CNN detectors in total and formed the set of victim %forensic CNN detectors 
classifiers we attacked in this paper.  


\begin{comment}
\begin{table}[!t]
\centering
\caption{The number of GAN-generated images  in the \textit{Eval-set} of the object dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|cccccc}
\textbf{GANs}& ProGAN&CycleGAN& StyleGAN& StyleGAN2& BigGAN& GauGAN\\
\hline
\textbf{No. of images} &4,000 & 1,300 &6,000 &8,000 &2,000 &5,000\\
\end{tabular}}
\label{tab: set1}
\end{table} 
%\vspace{2em}
\end{comment}

%%
All CNN detectors were trained from scratch for 20 epochs on both datasets.   
%
The input size of each CNN was a $256\times 256$ image.  
For images of resolution $1024\times 1024$,  we randomly cropped a $256\times 256$ pixel patch from each image during training and testing. % the detectors.
%
%%  
We chose the set of hyperparameters for each CNN  that yielded the highest classification accuracy after a grid search.  For Xception the learning rate started at $0.01$;  for ResNet-50 the learning rate started at $0.0001$ and for all other CNNs the learning rate started at $0.0005$.  These learning rates decayed by half every 4 epochs.  Weights were initialized using Xavier initializer~\cite{xavier}, biases were initialized as $0$'s, and both were optimized using stochastic gradient descent.  


To benchmark the performance of the victim CNN detectors,  we calculated the classification accuracy achieved by each CNN detector. The classification accuracy is defined as the percentage of the real and GAN-generated images that were correctly classified by the CNN detector out of  all images in \textit{Eval-set}.   
%
%
The classification accuracy achieved by each victim CNN detector on  both datasets are shown in Table~\ref{tab: acc}.  On average,  we achieved $95.94\%$ classification accuracy on the human face dataset and $99.14\%$ classification accuracy on the object dataset.   The results showed that the CNN detectors used  in this paper were not biased.  

\begin{table}[!t]
\centering
\caption{Baseline classification accuracies of the victim CNN detectors achieved on the human face dataset and  the object dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c||c}
\hline
\textbf{CNNs} &\textbf{ Human Face Dataset}&  \textbf{Object Dataset}\\
\hline
\textbf{Xception} &99.67\%&99.75\% \\
\textbf{ResNet-50}& 78.26\%&99.14\%\\
\textbf{DenseNet} &96.39\%&97.04\%\\
\textbf{MISLNet}& 99.93\%&99.15\%\\
\textbf{PHNet} & 95.15\%&99.73\%\\
\textbf{SRNet} &99.50\% &99.78\%\\
\textbf{Image CNN}& 99.49\% & 99.10\%\\
\textbf{CamID CNN} & 99.16\%& 99.46\%\\
\textbf{Avg.}&\textbf{95.94\%} & \textbf{99.14\%}\\
\hline
\end{tabular}}
\label{tab: acc}
\end{table}
 
 \begin{comment}
Additionally,  since the goal of this paper is to attack GAN-generated images and  fool CNN detectors,  we wanted to compare the performance of the victim CNN detectors on classifying GAN-generated images before and after the attack being launched.   To do this,  we calculated the recalls of classifying GAN-generated images.  The recall associated with one particular pair of CNN detector and GAN method is defined as the percentage of the GAN-generated images that were correctly detected by the CNN detector out of the generated images produced by that GAN method. 

Table~\ref{tab: recall_face} shows the recalls achieved by each victim CNN detector on the  human face dataset.  Each entry is associated with one victim CNN detector and  one  GAN method.  The average recall achieved on the human face dataset is  $ 94.53\%$.   The recall on classifying StarGAN-v2 generated image is $98.66\%$,  on classifying StyleGAN generated images is $92.15\%$,  and on classifying StyleGAN2 generated image is $92.77\%$.  The results showed that the CNN detectors can reliably detect GAN-generated images of human faces before the attack being launched. 

Table~\ref{tab: recall_object} shows the recalls  achieved by each victim CNN detector on the object dataset.  Each entry is associated with one victim CNN detector and  one  GAN method.  The average recall achieved on the object dataset is   $77.12\%$.  The results are consistent with previous research by Wang et al. ~\cite{wang2020cnn},  and showed that the CNN detectors can reliably detect GAN-generated images of objects  before the attack being launched. 

The baseline performance of the victim forensic CNN detectors demonstrated  that  CNN detectors used in this paper were well-trained,  and can be used  to evaluate the proposed attack in the following experiments. 



\begin{table}[!t]
\centering
\caption{Recalls of detecting GAN-generated images of human faces by the victim forensic CNN detectors. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{CNNs} & \textbf{StarGAN-v2} &\textbf{StyleGAN} &\textbf{StyleGAN2}&\textcolor{blue}{\textbf{Avg.}}\\
\hline
\textbf{Xception}&99.92\% & 99.90\%&100.00\% &99.94\%\\
\textbf{ResNet-50}&95.65\% & 49.12\% & 67.62\%&70.80\%\\
\textbf{DenseNet} &98.40\%&96.27\% &99.22\% &97.96\%\\
\textbf{MISLNet}&99.95\%  &99.97\% &100.00\%&99.97\%\\
\textbf{PHNet} & 97.37\% & 93.65\% &76.00\%&89.01\%\\
\textbf{SRNet}  & 99.27\%& 99.75\% &99.80\%&99.61\%\\
\textbf{Image CNN}& 99.95\% &99.12\% &99.90\%&99.66\%  \\
\textbf{CamID CNN} &98.77\% &99.42\% & 99.65\%&99.28\%\\
\textcolor{blue}{\textbf{Avg.}}& \textcolor{blue}{\textbf{98.66\%}}& \textcolor{blue}{\textbf{92.15\%}}&\textcolor{blue}{\textbf{92.77\%}}&\textcolor{blue}{\textbf{94.53\%}}\\
\hline
\end{tabular}}
\label{tab: recall_face}
\end{table}


\begin{table} [!t]
\centering
\caption{Recalls of detecting GAN-generated images of objects by the victim forensic CNN detectors.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textcolor{blue}{\textbf{Avg. }}\\
\hline
\textbf{Xception}&99.82\%&69.56\% &70.92\% & 72.91\% &19.61\%& 34.50\%&61.22\%\\
\textbf{ResNet-50} &99.65\%& 77.08\% &77.06\% & 92.41\% &82.40\% &82.29\%&85.15\%  \\
\textbf{DenseNet}&96.90\% & 77.70\%&61.98\% &88.69\% &78.75\% & 80.93\%&80.83\%\\
\textbf{MISLNet}&98.80\% & 73.16\%& 89.59\%&78.14\% & 73.05\% & 34.45\%&74.53\% \\
\textbf{PHNet} &99.78\% &65.34\% &76.34\%& 89.61\%&79.80\%&57.49\%&78.06\%\\
\textbf{SRNet} &99.72\%& 100.00\% &69.68\% & 33.50\%& 99.85\%&99.76\%& 83.75\%\\
\textbf{Image CNN}&99.90\% &41.89\% & 92.97\%& 97.40\% &86.35\% &80.40\%&83.15\%\\
\textbf{CamID CNN} & 99.70\%& 43.54\% & 71.37\% & 79.53\% & 68.25\%&59.31\%&70.28\% \\
\textcolor{blue}{\textbf{Avg.}} &\textcolor{blue}{\textbf{99.28\%}}&\textcolor{blue}{\textbf{68.53\%}}&\textcolor{blue}{\textbf{76.24\%}}&\textcolor{blue}{\textbf{79.02\%}}&\textcolor{blue}{\textbf{73.51\%}}&\textcolor{blue}{\textbf{66.14\%}}&\textcolor{blue}{\textbf{77.12\%}}\\
\hline
\end{tabular}}
\label{tab: recall_object}
\end{table}
\end{comment}

%\subsection{Attack Evaluation Metrics}
%A successful anti-forensic attack should be able to fool forensic CNN detectors with high probability,  and maintain high visual quality.   We used the following metrics  to evaluate the  proposed  attack on fooling the CNN detectors and the visual quality of the attacked images. 

%\subhead{Attack Success Rate} To evaluate the performance of the proposed attack in terms of  fooling  the victim CNN detectors,  we define the  attack success rate  as the percentage of the attacked images that are classified as ``real" by the victim CNN detector.

%\subhead{Image Quality} To  evaluate the visual quality of  attacked images produced by the proposed attack,  we calculated the mean PSNR and mean SSIM between the  GAN-generated images and the attacked images. 


\subsection{White-Box Attack}
The first set of experiments was designed to evaluate the effectiveness of our proposed attack in the white-box scenario.  Here,  we assume the attacker has access to the victim classifier and can train directly against it.

%In the white-box scenario,  we assume the attacker has access to the victim CNN detector.   Therefore,  the attacker can train an anti-forensic generator directly against the victim  CNN detector he/she is attempting to fool. 

For  each victim CNN detector trained on the  human face dataset and the object dataset,   we trained an individual anti-forensic generator to attack it.  To evaluate the performance of the anti-forensic generator,  we used the generator to attack each GAN-generated image in the \textit{Eval-set},   saving the attacked images to  disk as PNG files.   This is to ensure the pixel values of  attacked images reside in the range from 0 to 255.   Next,  we calculated the attack success rate  by using the victim CNN detector  to classify the attacked images.  We also calculated the mean PSNR and mean SSIM between the GAN-generated images and the attacked images to evaluate the visual quality of the attacked images.  

%%%
The anti-forensic generators presented in this paper were trained from scratch for 32 epochs with a learning rate of $0.0001$.  
Weights were initialized using Xavier initializer~\cite{xavier} and biases were initialized as $0$'s, and were optimized using stochastic gradient descent. 
%Weights and biases were optimized using stochastic gradient descent.   
%
To balance the image  quality and attack success rates,  $\alpha$ in equation~\ref{eq:g_loss} was chosen after a grid search range from $1$ to $200$ with an increment of $20$.  Specifically,  $\alpha$ was chosen to be $20$ 
for attacks on the human face dataset and $100$ for attacks on the object dataset. 
%when attacking the victim CNN detectors trained  on the  human face dataset and $\alpha$ was chosen to be $100$ when  attacking victim CNN detectors trained on the object dataset.  
When training our attack on the human face dataset, we randomly cropped $256\times 256$  patches from images of size $1024\times 1024$.



\subsection{Zero-Knowledge Attack}
This set of experiments was conducted to evaluate the proposed attack in the zero-knowledge scenario.  We assume the attacker has no knowledge about the victim CNN detector that the investigator would use to classify images.  Particularly,  the attacker has no access to the victim CNN detector and cannot observe any input or output of the CNN detector,  since the investigator may use a private CNN detector that the attacker by all means cannot have access to.   This is a more realistic yet challenging scenario. 
In the zero-knowledge scenario,   we evaluated the transferability of the proposed attack to attack unseen CNN detectors.  

To achieve the transferability,  we built an ensemble of forensic CNN detectors to train the proposed anti-forensic generator.   To mimic the zero-knowledge scenario,   each ensemble used to train the %proposed
attack did not include 
%the CNN detector used for evaluating the attack.
the victim classifier.  
 We assume that if the attacker has no knowledge of the % CNN detector
 victim classifier's architecture,  
%the attacker will use all available CNN detectors to make the attack as strong as possible.    
the attacker will use  all available CNNs in their ensemble to strenthen their attack.   
%However,  due to the limitation of computer memory,  the Xception was always excluded from the ensemble when attacking other networks.  
However,  due to limited GPU memory,  Xception was always excluded from the training ensemble in our experiments. 
During training,  we used the same hyperparameters and other settings as the white-box scenario. 







==> sections/intro_v0.tex <==
%introduction_v0





Recent technological advances have enabled the creation of synthetic images that are visually realistic.  Generative adversarial networks (GANs) in particular have driven this development.  
%Several GANs have been proposed that are capable of creating visually plausible images of both objects and human faces
Several GANs have been proposed that are capable of synthetically generating images of both objects~\cite{ } and human faces~\cite{ } that are convincingly real to human observers. 
Unfortunately, these synthetic image generation techniques can be used for malicious purposes, such as the creation of fake personas to be used as part of misinformation campaigns~\cite{ }.


To combat this threat, researchers have developed a variety of techniques to detect GAN-generated imagery~\cite{cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn}  
and to attribute synthetic images to the specific GAN used to create them~\cite{marra2019, 9035099, 9010964}.
%and  to identify the specifc GAN used for  images~\cite{marra2019, 9035099, 9010964}.
Importantly, work by Wang et al. showed that a convolutional neural network (CNN) trained to identify synthetic images can also detect images made by GANs not seen during training~\cite{wang2020cnn}.



%Previous research has shown that GAN-generated images left forensic traces that are very distinguishable from real images\cite{cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn,marra2019, 9035099,9010964}.   Forensic algorithms have been designed to detect GAN-generated imagery~\cite{cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn},  and  identify identifying specifc GAN used for generating images~\cite{marra2019, 9035099, 9010964}.   Recent research by Wang et al. ~\cite{wang2020cnn} shows that CNN can be trained  as the detector and learn  general underlying forensic  traces left by synthesized images.   By training an ResNet-50 to differentiate real images and ProGAN generated images,  this image detector can identify synthesized images created by other generative methods ,  including six GAN-based generative methods.  

At the same time, adversarial examples have arisen as a new threat to classifiers built from neural networks~\cite{ }.  A variety of different techniques have been proposed to generate adversarial examples~\cite{}.  These represent important threats to the forensic community because they can be used as an anti-forensic attack against forensic detectors~\cite{ }.   
%In a similar vein, GAN-based approaches have also been proposed to create deep-learning-based anti-forensic attacks~\cite{ }. 
Recent work from the forensic community, however, suggests that these attacks may not achieve transferability, i.e. they may be unable to attack classifiers other than those that they were directly trained against.  
%This is an important difference from attacks against classifiers used in computer vision.
%, unlike attacks demonstrated in the computer vision community.


%For an anti-forensic attack to be successful, it must fool a victim classifier and maintain high visual quality within the attacked image.  Furthermore, it is highly desirable for an attack to transfer to victim classifiers not seen  during training and be easily deployable in practical scenarios, i.e. it should work on images of any size, not require specific knowledge of the image window analyzed by a forensic CNN, deploy quickly and efficiently, etc.


For an anti-forensic attack to be successful, it must (1)~fool a victim classifier and (2) maintain high visual quality within the attacked image.  Furthermore, it is highly desirable for an attack to (3) transfer to victim classifiers not %encountered 
seen  during training and (4) be easily deployable in practical scenarios, i.e. it should work on images of any size, not require specific knowledge of the image window analyzed by a forensic CNN, deploy quickly and efficiently, etc.

%At the same time adversarial examples have arisen,  and they are starting to be used as anti-forensic attacks. Carlini and Farid ~\cite{carlini2020evading} showed

\begin{comment}
 For an attack to be successful it must
 (1) Fool a classifier
(2) Maintain high image quality
For optimal (highly desirable) results, it should also:
(3) Transfer if possible
(4) work in practical scenarios
  (a) work on any image size
  (b) not require knowledge of the blocking grid
  (c) deploy quickly and efficiently,  image-idependent 
\end{comment}


%While adversarial examples can achieve some of these goals, room for improvement exists. 

In this paper, we propose a new attack that is capable of fooling forensic synthetic image detectors into thinking that {\gi}s are in fact real images.  
This attack achieves each of the four goals described above, including a significant degree of transferability,  which enables it to attack victim classifiers that are unseen during training.  
%
Instead of crafting adversarial examples that exploit flaws in forensic deetctors, our attack uses an \ag to synthesize forensic traces associated with real images.  We propose GAN-based approaches for training our \ag for both white box scenarios as well as zero-knowledge scenarios.  
%We achieve transferability in zero-knowledge scenarios by training against
%We propose two GAN-based training procedures for our \ag; one for white box scenarios and one for zero-knowledge scenarios.  
Once the \ag is trained,  it can be used to attack images of arbitrary size without requiring re-training or additional tuning to the image under attack.



%In this paper we propose a new attack that takes an different approach from adversarial example attacks.  Instead of crafting adversarial examples that exploits the flaws of CNN detectors,  we propose to falsify forensic traces of GAN-generated images corresponding to real images,  such that the attacked images produced by our proposed attack will be classified as ``real" by  synthetic image CNN detectors.  Our attack operates by first train an an-forensic generator adversarially against forensic CNNs to learn the forensic traces of real images,   and then used the trained generator to attack GAN-generated images.   Once the anti-forensic generator is trained,  it can be applied to images of arbitrary sizes

The main contributions of this work are as follows:
\begin{itemize}
\vspace{-0.5em}
\setlength\itemsep{0.0em}
\item We demonstrate that an anti-forensic generative attack can be used to fool forensic CNNs designed to detect {\gi}s.

%We demonstrate that a generative attack can be used to fool forensic CNNs trained to detect GAN generated images.  

\item  We propose a new anti-forensic generator architecture that is able to synthesize forensic traces associated with real images while introducing no perceptible distortions into an attacked image.  We show that our proposed generator architecture yields important performance improvements over existing {\ag}s in terms of both attack success rate and image quality.

\item  We propose an ensemble loss training strategy that enables our attack to achieve transferability in zero-knowledge scenarios.

\item We demonstrate the effectiveness of our attack against many state-of-the-art forensic CNNs, using a synthetic images from a wide variety of different GANs.
\end{itemize}

==> sections/intro_v1-short.tex <==
%intro_v1-short

Recent technological advances have enabled the creation of synthetic images that are visually realistic.  Generative adversarial networks (GANs)~\cite{GAN2014} in particular have driven this development.  
%Several GANs have been proposed that are capable of creating visually plausible images of both objects and human faces
Several GANs have been proposed that are capable of synthetically generating images of both objects and human faces that are convincingly real to human observers~\cite{starganv2choi2020, stylegan2Karras2019, stylegankarras2019style,  bigganbrock2018large,gauganpark2019gaugan,progankarras2017progressive,  choi2018stargan}. 
Unfortunately, these synthetic image generation techniques can be used for malicious purposes, such as the creation of fake personas to be used as part of misinformation campaigns.


To combat this threat, researchers have developed many techniques to detect GAN-generated images~\cite{cozzolino2018forensictransfer,  mccloskey2018detecting,  nataraj2019detecting, zhang2019detecting, wang2020cnn}  
and to attribute them %synthetic images 
to the specific GAN used to create them~\cite{marra2019, 9035099, 9010964}.
%Importantly, work by Wang et al. showed that a convolutional neural network (CNN) trained to identify synthetic images can also detect images made by GANs not seen during training~\cite{wang2020cnn}.
%
%
%
At the same time, adversarial examples have arisen as a new threat to classifiers built from neural networks~\cite{L-BFGS,fgsm,iterative-fg,jsma,cw,pgd}.  
%A variety of different techniques have been proposed to generate adversarial examples~\cite{}.  
These represent important threats to the forensic community because they can be used as an anti-forensic attack against forensic detectors~\cite{barni2018adversarial,carlini2020evading,counter2017CNN}.   
%In a similar vein, GAN-based approaches have also been proposed to create deep-learning-based anti-forensic attacks~\cite{ }. 
Recent work from the forensic community,  however, suggests that these attacks may not achieve transferability,  i.e. they may be unable to attack classifiers other than those  they were directly trained against~\cite{transferability_Barni,zhao2020effect}.  
%This is an important difference from attacks against classifiers used in computer vision.
%, unlike attacks demonstrated in the computer vision community.


%For an anti-forensic attack to be successful, it must fool a victim classifier and maintain high visual quality within the attacked image.  Furthermore, it is highly desirable for an attack to transfer to victim classifiers not seen  during training and be easily deployable in practical scenarios, i.e. it should work on images of any size, not require specific knowledge of the image window analyzed by a forensic CNN, deploy quickly and efficiently, etc.


For an anti-forensic attack to be successful,  it must (1)~fool a victim classifier and (2) maintain high visual quality within the attacked image.  Furthermore, it is highly desirable for an attack to (3) transfer to victim classifiers not %encountered 
seen  during training and (4) be easily deployable in practical scenarios, i.e. it should work on images of any size, not require specific knowledge of the image window analyzed by a forensic CNN, deploy quickly and efficiently, etc.


In this paper, we propose a new attack that is capable of fooling forensic synthetic image detectors into thinking that {\gi}s are in fact real images.  
This attack achieves each of the four goals described above,  including a significant degree of transferability,  which enables it to attack victim classifiers that are unseen during training.  
%
Instead of crafting adversarial examples that exploit flaws in forensic detctors,  our attack uses an \ag to synthesize forensic traces associated with real images.  We propose GAN-based approaches for training our \ag for both white-box scenarios and zero-knowledge scenarios.  
%We achieve transferability in zero-knowledge scenarios by training against
%We propose two GAN-based training procedures for our \ag; one for white box scenarios and one for zero-knowledge scenarios.  
Once the \ag is trained,  it can be used to attack images of arbitrary size without requiring re-training or additional tuning to the image under attack.


The main contributions of this work are as follows:
\begin{itemize}
%\vspace{-0.5em}
%\setlength\itemsep{0.0em}
\setlength\itemsep{-0.2em}
\item We demonstrate that an anti-forensic generative attack can be used to fool forensic CNNs designed to detect {\gi}s.

%We demonstrate that a generative attack can be used to fool forensic CNNs trained to detect GAN generated images.  

\item  We propose a new anti-forensic generator %architecture 
that is able to synthesize forensic traces associated with real images while introducing no perceptible distortions into an attacked image.  We show that our proposed generator % architecture 
achieves in a higher attack success rate and image quality than  other alternative attacks.
%yields important performance improvements over existing {\ag}s in terms of both attack success rate and image quality.

\item  We propose an ensemble loss training strategy that enables our attack to achieve transferability in zero-knowledge scenarios.

\item We demonstrate the effectiveness of our attack against many state-of-the-art forensic CNNs,  using synthetic images from a wide variety of different GANs.
\end{itemize}

==> sections/proposed.tex <==
% proposed
\section{Proposed Adversarial Generator Attack}
\subsection{Overivew}

In this paper, we attempt to launch an attack to  forge forensic traces of  GAN-generated images,  such that attacked images will be classified as "real" by forensic CNN detectors.  To do this,  we propose to use  an adversarial generator that takes in a GAN-generated image,  remove the forensic traces left by GANs,  introduce forensic traces that corresponds to ``real",  and produces an attacked image.    The attacked image proposed by the proposed attack has the same contents as the GAN-generated image,  maintain a high perceptual quality and can fool forensic CNN detectors. 
The generator is adversarially trained using a GAN to learn forensic traces of real images.  The proposed attack is image-independent.  During deployment,  the proposed attack can be applied to any GAN-generated images of arbitrary sizes.   Additionally,  we propose two training protocols for  white-box attack and zero knowledge attack.  

\begin{comment}
can fool forensic CNNs  trained for detecting GAN-generated images.  To do this,  we propose a new attack that utilize a GAN to construct an adversarial generator that were trained explicitly to learn the forensic traces of real images.  The adversarial generator takes in an GAN-generated image,  synthesize its forensic traces,   and produce a crafted adversarial image.  The crafted adversarial images have the same content as the GAN-generated image. However,  the forensic CNN detector shall classify the adversarial  image as "real".  The adversarial images produces by the proposed attack not only is capable of fooling CNN detectors in the white-box scenarios,  but also demonstrate strong transferability when the attacker has zero knowledges about CNN architecture of the forensic CNNs detectors.    Additionally,  the proposed adversarial generator attack only introduces very minimal visual distortions that are barely perceptible to human eyes.

The overview of the proposed attack is shown in Figure~\ref{fig: proposed}.   The adversarial generator $G(\cdot)$ synthesizes forensic traces and produces an adversarial Image to fool the pretrained forensic CNN or the CNN ensemble.  The pre-trained forensic CNN or each CNN in the ensemble $C{\cdot}$  can validate if the adversarial images produced by the adversarial generator is successful or not,  and guide  the generator to mimic forensic traces of real images.  The training stops when the adversarial image can successfully fool the pretrained forensic  CNN or CNN ensemble and achieves high visual quality. 


\begin{figure}[!t]
\centering
\includegraphics[scale=0.4]{figures/proposed}
\caption{Overview of the propose attack}
\label{fig: proposed}
\end{figure}
\end{comment}


\subsection{Architecture of the Adversarial Generator}
The architecture of the proposed adversarial generator is shown in Figure~\ref{fig: generator} .  It consists of two consecutive convolutional blocks and a feature reduction layer.  A convolutional block is constructed with three identical convolutional layers followed by ReLU activation.   We used 64 filters in the  first convolutional block and 128 filters in the first convolution blocks.  The feature reduction layer is constructed with a convolutional layer followed by ReLU activation.  It reduces 128 feature maps to  three color layers.  All convolutional layers use $3\times 3$ filter with stride 1.  Small filter size allows the generator to synthesize  forensic traces in small areas,  and stride 1 ensures the generator produces attacked images  of the  same size as input image.   The output of the generator is the summation of the input of the generator and output of the feature reduction layer. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{figures/generator.pdf}
\caption{Architecture of the proposed adversarial  generator.}
\label{fig: generator}
\end{figure}


\subsection{Loss Function of the Adversarial Generator}
The loss function of the adversarial generator is formulated to ensure the generated adversarial images both can fool forensic CNN detectors and maintain high visual quality.   The  loss function $\mathcal{L}_{G}$ is formulated as the weighted sum of perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$ ,
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is the weight to balance the visual quality and performance of the attack. 

\underline{Perception loss} is to ensure the visual quality of the generated images produces by the adversarial generator.  It is calcualted as the mean absolute different between the GAN-generated image $I$ (i.e input of the generator ) and the adversarial images produced by the attack,  
\begin{equation}
\mathcal{L}_p =\frac{1}{w\times h}\sum_{\ell=1}^{3}\sum_{i=1}^{w}\sum_{j=1}^{h}\mid I_{i,j}-G(I)_{i,j}\mid,
\label{eq: perceptual_loss]}
\end{equation}
where $G(\cdot)$ represents the adversarial generator,  and subscripts $i, j$ represent the pixel's coordinates.

\underline{Classification loss} measures if  the  attacked images produces by the adversarial generator can fool the forensic CNN detector.  The formulation of classification loss depends on the attacker's knowledge level of the CNN detector.  We now individually discuss the formulation of classification loss  for the white-box attack and the zero knowledge attack. 

\begin{comment}
For a single CNN detector $C_s(\cdot)$ under attack,  the classification loss $\mathcal{L}_{c}^{(s)}$ is calculated as the softmax cross-entropy between the output of the CNN and the real class. 
\begin{equation}
\mathcal{L}_{c}^{(s)}=-\sum_{k=1}^{2} t_k \log\left(C_s(G(I))_k\right),
\label{eq: classification_loss}
\end{equation}
where $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ at the location of the unaltered class and $0$'s elsewhere. 
For the white-box attack,   the CNN detector is used for training the adversarial generator directly,  $\mathcal{L}_c=\mathcal{L}_c^{(s)}$.  For transferability in the zero knowledge scenario,  t
\end{comment}

\subsection{White-Box Attack Training}
In the white-box scenario,  the attacker has access to CNN detector to attack.   The adversarial generator can be directly trained against the forensic CNN detector under attack.  

For white-box attack,  the classification loss $\mathcal{L}_c$ is calculated as the softmax cross-entropy between the CNN detector's  output of attacked images and the real class. 

\begin{equation}
	\mathcal{L}_c =-\sum_{k=1}^{2} t_k \log\left(C(G(I))_k\right),
	\label{eq: white-box}
\end{equation}
where $C(\cdot)$ represent the CNN detector to attack,  $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ for the real class and a $0$ for the fake class.

\subsection{Zero Knowledge Attack Training}
In the zero knowledge scenario,  the attacker has no knowledge about the CNN detector to attack.  Particularly,  the attacker has zero knowledge of the architecture of the CNN detector.  The attacker cannot observe any inputs and outputs of the CNN detector.   It requires the proposed attack achieve transferability to fool other CNN detectors unseen by the adversarial generator.  To achieve the transferability,  we propose to use the ensemble of CNN detectors available to the attacker to train the adversarial generator.  The intuition of the CNN ensemble is that each  CNN detector learns an aspect of forensic traces of real images,  and form a unique boundary of real class,  hence the ensemble of forensic CNN detectors can guide  the generator to learn a  comprehensive information of real images.  If the generated adversarial  image can fool each CNN  detector in the ensemble,  it most likely can fool unseen CNN detectors. 

For the zero knowledge attack,  the classification loss $\mathcal{L}_c$ is  formulated as the weights sum of individual classification loss pertaining to each CNN detector in the ensemble, 
\begin{equation}
\mathcal{L}_c= \sum_{s=1}^{S} \beta^{(s)} \mathcal{L}_c^{(s)}
\end{equation}
where $S$ is the number of CNN detectors in the ensemble, $ \mathcal{L}_c^{(s)}$ corresponds to individual classification loss of the $s^{th}$ CNN detector calculated using Equation~\ref{eq: white-box},  $\beta^{(s)}$ corresponds to the weight of  $s^{th}$ individual classification loss. 


\begin{comment}
\subhead{The Pretrained Forensic CNN (Ensemble)}  The goal of the pretrained forensic CNN or CNN ensembles is to enforce the adversarial generator to learn the forensic traces of real images.  Previous research shows that GANs leaves unique forensic traces and are different from real images~\cite{wang2020cnn}. The  CNN  or each CNN in the ensemble is a forensic detector,   a binary classifier of real and fake(i.e GAN-generated) classes.  The CNN detectors are pre-trained and are not updated during training the adversarial generator. 
In the white box scenario,  the pre-trained forensic CNN is the CNN detector the attacker aimed to fool.   If the attacker has zero knowledge about the forensic CNN detector the investigator uses,  the attacker can form a CNN ensemble using forensic CNN detectors of his/her own and incorporate the ensemble to train the adversarial generator.  The goal of CNN ensemble is to achieve transferability and fool CNN not seen by the adversarial generator. 
\end{comment}

\subsection{Image-Independent Attack}
Once trained,  the proposed adversarial generator is image-independent.  The trained adversarial generator can attack any image of arbitrary sizes and doesn't need to retrain the attack.   To launch the attack,  the attacker can use the adversarial generator to attack full-size color image at once.  If the attacker does not possess enough computational resources to attack full-size images at once,  the attacker can divide the full-size color image into smaller patches and use the generator to attack each image patch individually,  and then group the anti-forensically attacked patches together in the original order to form the full-size attacked image.

The proposed attack is agnostic to blocking artifacts.  Most of CNN detectors operates on predicting patches of an image.  Even though the attacker does not know which patch may be used for detection,  the attacker can simply apply the attack on the full-size image and any patch from the attacked image can still fool the CNN detector. 




 


==> sections/proposed_v2.tex <==
% proposed
\section{Proposed Attack}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
We note that this attack is different from adversarial example generation algorithms % developed in machine learning literature  
such as FGSM, PGD, or CW~\cite{ } in several important ways.  

These algorithms all approximately operate by creating pertubations $\delta$ that are added to an image in order to fool a classifier.  The adversarial perturbations $\delta$ are the same size as the input to the victim classifier.  %, and are iteratively learned by 
They are learned through an iterative process in which an intermediate version of the attacked image is presented to the victim classifier, gradient information is inferred, and the attack pertubation is updated.  As a result, a new perturbation must be iteratively learned for each image under attack.

By contrast our attack learns a convolutional generator which is trained in advance.   The generator is not modified or customized to the image under attack.   Any image of arbitrary size can be passed through the generator, not just images with the same size as the victim CNN's input.  

Most importantly, our attack differs philosophically from adversarial examples.  Adversarial examples aim to find minor perturbations that cause a victim classifier to misclassify an input.  Several explanations as to why adversarial examples exist, including 
imperfections caused by the locally-linear nature of neural networks 
%% [11] - Goodfellow, Ian J., Jonathon Shlens, and Christian Szegedy. "Explaining and harnessing adversarial examples." arXiv preprint arXiv:1412.6572 (2014).
or that there is misalignment between the features used by humans and those learned by neural networks when performing the same classification task.
% Adversarial Examples Are Not Bugs, They Are Features
%
%  They accomplish this goal by exploiting ``blind spots'' that occur due to %inadequate training or overfitting to t

Our attack instead aims to accurately synthesize forensic features used by a CNN, that are otherwise used to \textit{correctly} classify that image.  


Our attack does intend to exploit adversarial perturbations that may clause a neural network to misclassify an input.  Instead, our attack aims to accurately synthesize the forensic features that are used are used to \textit{correctly} classify an unattacked image. 
%
When doing this, we are able to exploit the fact that forensic traces are not visible to the human eye.  As a result, we can completely falsify these traces without modifying the contents of an image.  We believe that this is the key to the improved transferability of our attack.  
%We note, however, that this approach may not work against classifiers for computer vision tasks because 

%This approach may not be possible 



%%%%%%%% WRITING NOTE %%%%%%%%
%From Carlini & Wagner, "Towards Evaluating the Robustness of Neural Networks"
%The key insight here is that by training to match the first network, we will hopefully avoid over-fitting against any of the training data. If the reason that neural networks exist is because neural networks are highly non-linear and have “blind spots” [46] where adversarial examples lie, then preventing this type of over-fitting might remove those blind spots.
%
% REFERENCE [46] - SZEGEDY, C., ZAREMBA, W., SUTSKEVER, I., BRUNA, J., ERHAN, D., GOODFELLOW, I., AND FERGUS, R. Intriguing properties of neural networks. ICLR (2013).
%
%
% IIn fact, as we will see later, defensive distillation does not remove adversarial examples. One potential reason this may occur is that others [11] have argued the reason adversarial examples exist is not due to blind spots in a highly non-linear neural network, but due only to the locally-linear nature of neural networks. This so-called linearity hypothesis appears to be true [47], and under this explanation it is perhaps less surprising that distillation does not increase the robustness of neural network
%
% [11] - Goodfellow, Ian J., Jonathon Shlens, and Christian Szegedy. "Explaining and harnessing adversarial examples." arXiv preprint arXiv:1412.6572 (2014).

% Adversarial Examples Are Not Bugs, They Are Features

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Overivew}


%Our attack operates by using an attack generator to modify the forensic traces in a GAN-generated image, such that the attacked image will be classified as real by a forensic CNN .



%Our attack operates by using an \ag to falsify the forensic traces in a GAN-generated image so that a victim forensic classifier misidentifies the image as `real'.  The 


%Our attack is designed to modify a \gi such that it will fool a forensic CNN into misclassifying it as a `real' image.  

Our attack is designed to modify a \gi $I$ so that a forensic CNN will instead classify it as a `real' image.  
This forensic CNN is alternately referred to as the victim classifier, and is trained to differentiate between real and {\gi}s.


Our attack operates by passing the  \gi %GAN-generated image 
through a pre-trained \ag $G$ in order to falsify its forensic traces.  The \ag  is designed to remove forensic traces associated with {\gi}s and synthesize traces associated with `real' images.  
%
%As a result, a victim classifier, i.e. a forensic classifier that will be fooled by this attack, will misclassify the attacked GAN-generated image as a real one.
As a result, a victim classifier will %misclassify 
classify 
the attacked \gi $G(I)$ as a real one.
%
Furthermore, the \ag designed to make no changes to the image's contents and to introduce no visually perceptible distortions into the attacked image.  This will prevent a human from visually identifying that an image was attacked.  


The \ag in our attack learns to synthesize 'real' forensic traces through adversarial training.   %The \ag 
It is trained as part of a GAN in which the discriminator is replaced by a forensic classifier (or set of classifiers) that has been pre-trained to learn the distribution of forensic features associated with real and {\gi}s.  

Different  strategies are used to train the \ag depending on whether the attack is launched in a white box or zero-knowledge scenario. 
%
In the white box scenario, our attack aims to synthesize forensic features with the distribution learned by the victim classifier, even if they deviate from the ideal feature distribution of real images.
%distribution of features associated with real images.
In the zero-knowledge scenario, our attack aims to learn the  distribution of forensic features of real images.  However it avoids synthesizing features in regions where different classifiers may %use different decision boundaries.  
make different decisions.  
Instead, it aims to synthesize features that any classifier will likely associate with a real image. 


We  note that once our \ag is trained, our attack can be launched against any image without retraining.  Furthermore, since our attack is based on a convolutional generator, we can attack images of any size without the need to modify our generator or attack structure.  This differs from adversarial example generation techniques, which iteratively learn unique perturbations for each image that are the same size as the victim classifier's input.


In the following subsections, we provide detailed information about how our attack is built and deployed.




%In this paper, we attempt to launch an attack to  forge forensic traces of  GAN-generated images,  such that attacked images will be classified as "real" by forensic CNN detectors.  To do this,  we propose to use  an adversarial generator that takes in a GAN-generated image,  remove the forensic traces left by GANs,  introduce forensic traces that corresponds to ``real",  and produces an attacked image.    The attacked image proposed by the proposed attack has the same contents as the GAN-generated image,  maintain a high perceptual quality and can fool forensic CNN detectors. 
%
%The generator is adversarially trained using a GAN to learn forensic traces of real images.  The proposed attack is image-independent.  During deployment,  the proposed attack can be applied to any GAN-generated images of arbitrary sizes.   Additionally,  we propose two training protocols for  white-box attack and zero knowledge attack.  

\begin{comment}
can fool forensic CNNs  trained for detecting GAN-generated images.  To do this,  we propose a new attack that utilize a GAN to construct an adversarial generator that were trained explicitly to learn the forensic traces of real images.  The adversarial generator takes in an GAN-generated image,  synthesize its forensic traces,   and produce a crafted adversarial image.  The crafted adversarial images have the same content as the GAN-generated image. However,  the forensic CNN detector shall classify the adversarial  image as "real".  The adversarial images produces by the proposed attack not only is capable of fooling CNN detectors in the white-box scenarios,  but also demonstrate strong transferability when the attacker has zero knowledges about CNN architecture of the forensic CNNs detectors.    Additionally,  the proposed adversarial generator attack only introduces very minimal visual distortions that are barely perceptible to human eyes.

The overview of the proposed attack is shown in Figure~\ref{fig: proposed}.   The adversarial generator $G(\cdot)$ synthesizes forensic traces and produces an adversarial Image to fool the pretrained forensic CNN or the CNN ensemble.  The pre-trained forensic CNN or each CNN in the ensemble $C{\cdot}$  can validate if the adversarial images produced by the adversarial generator is successful or not,  and guide  the generator to mimic forensic traces of real images.  The training stops when the adversarial image can successfully fool the pretrained forensic  CNN or CNN ensemble and achieves high visual quality. 


\begin{figure}[!t]
\centering
\includegraphics[scale=0.4]{figures/proposed}
\caption{Overview of the propose attack}
\label{fig: proposed}
\end{figure}
\end{comment}




\subsection{Difference From Adversarial Examples}
\input{sections/difference_from_adv_examples_v2}


\subsection{ Proposed Anti-Forensic Generator}
The proposed anti-forensic generator consists of a sequence of convolutional layers followed by ReLU activations~\cite{ReLU} shown in Figure~\ref{fig: generator}.   The first three convolutional layers use  64 filters,  the middle three convolutional layers use 128 filters,  and the final convolutional layer uses three filters to reduce the 128 feature maps to a three color channel image.  The output of the generator is the summation of the  input of the generator and the output of the last activated convolutional layer.  The skip connection is designed to give the generator  a better initialization for producing  high visual quality attacked images.
All convolutional layers use $3\times 3$ filter with stride 1.  The small filter size allows the generator to synthesize forensic traces in small areas.  We avoid using any pooling layers  to ensure that the output of the generator is of the same size as the input of the generator.  Therefore,  the proposed anti-forensic generator can be applied to images of arbitrary sizes,  and does not need to be trained  for images of different sizes individually.   This characteristic  makes the deployment of the proposed  anti-forensic generator efficient and quick.  

%Additionally,  the proposed generator does not demand too much memory.  It allows us to train the proposed anti-forensic generator against an ensemble of CNN detectors to achieve transferability in the zero knowledge scenario,  even with commercial GPUs.

We note that our proposed generator is intentionally lightweight.  This allows it to be  trained using widely available commercial GPUs.  This also enables it to be quickly deployed at attack time.  

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{figures/generator.pdf}
\caption{Architecture of the proposed anti-forensic generator.}
\label{fig: generator}
\end{figure}


%\subsection{Loss Function of the Adversarial Generator}
\subsection{Anti-Forensic Generator Training}

When adversarially training the \ag~$G$, we use a loss function 
%The loss function of the \ag is 
formulated to ensure that an attacked image can both fool a victim classifier and maintain high visual quality.  
This  loss function $\mathcal{L}_{G}$ consists of the weighted sum of two terms: the perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$, such that
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is used to balance the trade-off between the visual quality and performance of the attack. 


%%%%%%
%
\begin{comment}
The loss function of the adversarial generator is formulated to ensure the generated adversarial images both can fool forensic CNN detectors and maintain high visual quality.   The  loss function $\mathcal{L}_{G}$ is formulated as the weighted sum of perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$ ,
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is the weight to balance the visual quality and performance of the attack. 
\end{comment}
%
%%%%%%%

%^&*

%\underline{Perception loss} 
\subhead{Perceptual Loss} This term is used to minimize distortions introduced by the \ag and control the visual quality of the attacked image.  We define this term as  the mean absolute difference between the \gi $I$ (i.e the input of the generator ) and the attacked image produced by the produced by the generator $G(I)$, such that
\begin{equation}
\mathcal{L}_p = \,\tfrac{1}{N} \|I-G(I) \|_1,
\label{eq: perceptual_loss]}
\end{equation}
where $N$ is the number of pixels in $I$ and $G(I) $
  

\begin{comment}
is to ensure the visual quality of the generated images produces by the adversarial generator.  It is calcualted as the mean absolute different between the GAN-generated image $I$ (i.e input of the generator ) and the adversarial images produced by the attack,  
\begin{equation}
\mathcal{L}_p =\frac{1}{w\times h}\sum_{\ell=1}^{3}\sum_{i=1}^{w}\sum_{j=1}^{h}\mid I_{i,j}-G(I)_{i,j}\mid,
\label{eq: perceptual_loss]}
\end{equation}
where $G(\cdot)$ represents the adversarial generator,  and subscripts $i, j$ represent the pixel's coordinates.
\end{comment}


%\underline{Classification loss} 
\subhead{Classification Loss} This term is used to measure if  the  attacked images produced by the anti-forensic generator can fool the  CNN detector used for training.  It allows the generator to learn forensic traces learned by the CNN detectors.  For the white-box attack,  the classification loss is provided by the victim  classifier.   For the  zero knowledge attack,   the classification loss is provided by an ensemble of classifiers chosen by the attack. 

\begin{comment}
For a single CNN detector $C_s(\cdot)$ under attack,  the classification loss $\mathcal{L}_{c}^{(s)}$ is calculated as the softmax cross-entropy between the output of the CNN and the real class. 
\begin{equation}
\mathcal{L}_{c}^{(s)}=-\sum_{k=1}^{2} t_k \log\left(C_s(G(I))_k\right),
\label{eq: classification_loss}
\end{equation}
where $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ at the location of the unaltered class and $0$'s elsewhere. 
For the white-box attack,   the CNN detector is used for training the adversarial generator directly,  $\mathcal{L}_c=\mathcal{L}_c^{(s)}$.  For transferability in the zero knowledge scenario,  t
\end{comment}

\subsection{White-Box Attack Training}


In the white-box scenario, the attacker has direct access to the forensic CNN under attack.  As a result, the \ag can be directly trained against the victim classifier.  In this case, we define the classification
loss $\mathcal{L}_c$ as the softmax cross-entropy between the CNN detector's  output of attacked images and the real class.  Specifically,
\begin{equation}
	\mathcal{L}_c =-\sum_{k=1}^{2} t_k \log\left(C(G(I))_k\right),
	\label{eq: white-box}
\end{equation}
where $C(\cdot)$ is the victim classifier and  $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ for the real class and a $0$ for the fake class.  
%
Defining the classification loss in this manner incentivizes the \ag to learn the victim classifier's model of forensic features from real images.  %that correspond to real images.


%In the white-box scenario,  the attacker has access to CNN detector to attack.   The adversarial generator can be directly trained against the forensic CNN detector under attack.  






\subsection{Zero Knowledge Attack Training}

In the zero knowledge scenario, the attacker has no access to the victim classifier that they wish to attack, nor do they know its architecture.  This differs from the black box scenario in which the attacker can probe the victim classifier through an API, then observe the victim classifier's input-output relationship.  Instead, the attacker must rely entirely on the transferability of their attack to fool the victim CNN.

To achieve transferability, we propose adversarially training against an ensemble of forensic classifiers created by the attacker. 
%
Here, the classification loss $\mathcal{L}_c$ is formulated as the weights sum of individual classification loss pertaining to each CNN detector in the ensemble, 
\begin{equation}
\mathcal{L}_c= \sum_{s=1}^{S} \beta^{(s)} \mathcal{L}_c^{(s)}
\end{equation}
where $S$ is the number of CNN detectors in the ensemble, $ \mathcal{L}_c^{(s)}$ corresponds to individual classification loss of the $s^{th}$ CNN detector calculated using Equation~\ref{eq: white-box},  $\beta^{(s)}$ corresponds to the weight of  $s^{th}$ individual classification loss. 

 Each classifier in the ensemble learns to partition the forensic feature space into separate regions for real and {\gi}s.  By defining the classifier loss in this fashion, we incentivize the \ag to synthesize forensic traces that lie in the intersection of these regions.  This corresponds to features that all classifiers in the ensemble, and likely other classifiers not in the ensemble, associate with real images.  This suggests that the classifiers in this ensemble should have as diverse architectures as possible.

We note that this differs from adversarially training against an ensemble classifier.  An ensemble classifier fuses the decisions of several weak classifiers to form an accurate representation of the ideal classification boundary separating real from {\gi}s.  We wish to avoid generating features in regions near the ideal decision boundary, since many different classifiers will likely make different decision in this region.  By synthesizing features that \textit{all} classifiers in our ensemble agree are real, we move away from the ambiguous region near the ideal decision boundary and further into the space that likely corresponds to real images.  This likely comes at a price of causing greater distortion, but ideally provides greater transferrability of our attack's  generated features.





\begin{comment}
In the zero knowledge scenario,  the attacker has no knowledge about the CNN detector to attack.  Particularly,  the attacker has zero knowledge of the architecture of the CNN detector.  The attacker cannot observe any inputs and outputs of the CNN detector.   It requires the proposed attack achieve transferability to fool other CNN detectors unseen by the adversarial generator.  To achieve the transferability,  we propose to use the ensemble of CNN detectors available to the attacker to train the adversarial generator.  The intuition of the CNN ensemble is that each  CNN detector learns an aspect of forensic traces of real images,  and form a unique boundary of real class,  hence the ensemble of forensic CNN detectors can guide  the generator to learn a  comprehensive information of real images.  If the generated adversarial  image can fool each CNN  detector in the ensemble,  it most likely can fool unseen CNN detectors. 

For the zero knowledge attack,  the classification loss $\mathcal{L}_c$ is  formulated as the weights sum of individual classification loss pertaining to each CNN detector in the ensemble, 
\begin{equation}
\mathcal{L}_c= \sum_{s=1}^{S} \beta^{(s)} \mathcal{L}_c^{(s)}
\end{equation}
where $S$ is the number of CNN detectors in the ensemble, $ \mathcal{L}_c^{(s)}$ corresponds to individual classification loss of the $s^{th}$ CNN detector calculated using Equation~\ref{eq: white-box},  $\beta^{(s)}$ corresponds to the weight of  $s^{th}$ individual classification loss. 

\end{comment}

\begin{comment}
\subhead{The Pretrained Forensic CNN (Ensemble)}  The goal of the pretrained forensic CNN or CNN ensembles is to enforce the adversarial generator to learn the forensic traces of real images.  Previous research shows that GANs leaves unique forensic traces and are different from real images~\cite{wang2020cnn}. The  CNN  or each CNN in the ensemble is a forensic detector,   a binary classifier of real and fake(i.e GAN-generated) classes.  The CNN detectors are pre-trained and are not updated during training the adversarial generator. 
In the white box scenario,  the pre-trained forensic CNN is the CNN detector the attacker aimed to fool.   If the attacker has zero knowledge about the forensic CNN detector the investigator uses,  the attacker can form a CNN ensemble using forensic CNN detectors of his/her own and incorporate the ensemble to train the adversarial generator.  The goal of CNN ensemble is to achieve transferability and fool CNN not seen by the adversarial generator. 
\end{comment}

\begin{comment}

\subsection{Image-Independent Attack}
Once trained,  the proposed adversarial generator is image-independent.  The trained adversarial generator can attack any image of arbitrary sizes and doesn't need to retrain the attack.   To launch the attack,  the attacker can use the adversarial generator to attack full-size color image at once.  If the attacker does not possess enough computational resources to attack full-size images at once,  the attacker can divide the full-size color image into smaller patches and use the generator to attack each image patch individually,  and then group the anti-forensically attacked patches together in the original order to form the full-size attacked image.

The proposed attack is agnostic to blocking artifacts.  Most of CNN detectors operates on predicting patches of an image.  Even though the attacker does not know which patch may be used for detection,  the attacker can simply apply the attack on the full-size image and any patch from the attacked image can still fool the CNN detector. 
\end{comment}




 


==> sections/proposed_v3.tex <==
% proposed
\section{Proposed Attack}

\subsection{Overivew}

Our attack is designed to modify a \gi $I$ so that a forensic CNN will instead classify it as a `real' image.  
This forensic CNN is alternately referred to as the victim classifier, and is trained to differentiate between real and {\gi}s.

Our attack operates by passing the  \gi 
through a pre-trained \ag $G$ in order to falsify its forensic traces.  The \ag  is designed to remove forensic traces associated with {\gi}s and synthesize traces associated with `real' images.  
%
%As a result, a victim classifier, i.e. a forensic classifier that will be fooled by this attack, will misclassify the attacked GAN-generated image as a real one.
As a result, a victim classifier will  classify 
the attacked \gi $G(I)$ as a real one.
%
Furthermore, the \ag designed to make no changes to the image's contents and to introduce no visually perceptible distortions into the attacked image.  This will prevent a human from visually identifying that an image was attacked.  


The \ag in our attack learns to synthesize `real' forensic traces through adversarial training.   %The \ag 
It is trained as part of a GAN in which the discriminator is replaced by a forensic classifier (or set of classifiers) that has been pre-trained to learn the distribution of forensic features associated with real and {\gi}s.  

Different  strategies are used to train the \ag depending on whether the attack is launched in a white-box or zero-knowledge scenario. 
In the white-box scenario, our attack aims to synthesize forensic features with the distribution learned by the victim classifier, even if they deviate from the ideal feature distribution of real images.
%distribution of features associated with real images.
%
In the zero-knowledge scenario, our attack aims to learn the  distribution of forensic features of real images.  However it avoids synthesizing features in regions where different classifiers may %use different decision boundaries.  
make different decisions.  
Instead, it aims to synthesize features that any classifier will likely associate with a real image. 



We  note that once our \ag is trained, our attack can be launched against any image without retraining.  Furthermore, since our attack is based on a convolutional generator, we can attack images of any size without the need to modify our generator or attack structure.  This differs from adversarial example generation techniques, which iteratively learn unique perturbations for each image that are the same size as the victim classifier's input.


%In the following subsections, we provide detailed information about how our attack is built and deployed.



\subsection{Difference From Adversarial Examples}
\input{sections/difference_from_adv_examples_v2}


\subsection{ Proposed Anti-Forensic Generator}
The proposed anti-forensic generator consists of a sequence of convolutional layers followed by ReLU activations~\cite{ReLU} shown in Figure~\ref{fig: generator}.   The first three convolutional layers use  64 filters,  the middle three convolutional layers use 128 filters,  and the final convolutional layer uses three filters to reduce the 128 feature maps to a three color channel image.  The output of the generator is the summation of the  input of the generator and the output of the last activated convolutional layer.  The skip connection is designed to give the generator  a better initialization for producing  high visual quality attacked images.
All convolutional layers use $3\times 3$ filter with stride 1.  The small filter size allows the generator to synthesize forensic traces in small areas.  We avoid using any pooling layers  to ensure that the output of the generator is of the same size as the input of the generator.  Therefore,  the proposed anti-forensic generator can be applied to images of arbitrary sizes,  and does not need to be trained  for images of different sizes individually.   This characteristic  makes the deployment of the proposed  anti-forensic generator efficient and quick.  



We note that our proposed generator is intentionally lightweight.  This allows it to be  trained using widely available commercial GPUs.  This also enables it to be quickly deployed at attack time.  

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{figures/generator.pdf}
\caption{Architecture of the proposed anti-forensic generator.}
\label{fig: generator}
\end{figure}


%\subsection{Loss Function of the Adversarial Generator}
\subsection{Anti-Forensic Generator Training}

When adversarially training the \ag~$G$, we use a loss function 
%The loss function of the \ag is 
formulated to ensure that an attacked image can both fool a victim classifier and maintain high visual quality.  
This  loss function $\mathcal{L}_{G}$ consists of the weighted sum of two terms: the perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$, such that
\vspace{-0.5em}
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is used to balance the trade-off between the visual quality and performance of the attack. 


%%%%%%
%
\begin{comment}
The loss function of the adversarial generator is formulated to ensure the generated adversarial images both can fool forensic CNN detectors and maintain high visual quality.   The  loss function $\mathcal{L}_{G}$ is formulated as the weighted sum of perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$ ,
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is the weight to balance the visual quality and performance of the attack. 
\end{comment}
%
%%%%%%%

%^&*

%\underline{Perception loss} 
\subhead{Perceptual Loss} This term is used to minimize distortions introduced by the \ag and control the visual quality of the attacked image.  We define this term as  the mean absolute difference between the \gi $I$ (i.e the input of the generator ) and the attacked image produced by the generator $G(I)$, such that
\begin{equation}
\mathcal{L}_p = \,\tfrac{1}{N} \|I-G(I) \|_1,
\label{eq: perceptual_loss]}
\end{equation}
where $N$ is the number of pixels in $I$ and $G(I) $
  

\begin{comment}
is to ensure the visual quality of the generated images produces by the adversarial generator.  It is calcualted as the mean absolute different between the GAN-generated image $I$ (i.e input of the generator ) and the adversarial images produced by the attack,  
\begin{equation}
\mathcal{L}_p =\frac{1}{w\times h}\sum_{\ell=1}^{3}\sum_{i=1}^{w}\sum_{j=1}^{h}\mid I_{i,j}-G(I)_{i,j}\mid,
\label{eq: perceptual_loss]}
\end{equation}
where $G(\cdot)$ represents the adversarial generator,  and subscripts $i, j$ represent the pixel's coordinates.
\end{comment}


%\underline{Classification loss} 
\subhead{Classification Loss} This term is used to measure if  the  attacked images produced by the anti-forensic generator can fool the  CNN detector used for training.  It allows the generator to learn forensic traces learned by the CNN detectors.  For the white-box attack,  the classification loss is provided by the victim  classifier.   For the  zero-knowledge attack,   the classification loss is provided by an ensemble of classifiers chosen by the attack. 

\begin{comment}
For a single CNN detector $C_s(\cdot)$ under attack,  the classification loss $\mathcal{L}_{c}^{(s)}$ is calculated as the softmax cross-entropy between the output of the CNN and the real class. 
\begin{equation}
\mathcal{L}_{c}^{(s)}=-\sum_{k=1}^{2} t_k \log\left(C_s(G(I))_k\right),
\label{eq: classification_loss}
\end{equation}
where $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ at the location of the unaltered class and $0$'s elsewhere. 
For the white-box attack,   the CNN detector is used for training the adversarial generator directly,  $\mathcal{L}_c=\mathcal{L}_c^{(s)}$.  For transferability in the zero-knowledge scenario,  t
\end{comment}

\subsection{White-Box Attack Training}

In the white-box scenario, the attacker has direct access to the forensic CNN under attack.  As a result, the \ag can be directly trained against the victim classifier.  In this case, we define the classification
loss $\mathcal{L}_c$ as the softmax cross-entropy between the CNN detector's  output of attacked images and the real class.  Specifically,
\begin{equation}
	\mathcal{L}_c =-\sum_{k=1}^{2} t_k \log\left(C(G(I))_k\right),
	\label{eq: white-box}
\end{equation}
where $C(\cdot)$ is the victim classifier and  $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ for the real class and a $0$ for the fake class.  
%
Defining the classification loss in this manner incentivizes the \ag to learn the victim classifier's model of forensic features from real images.  %that correspond to real images.









\subsection{Zero-Knowledge Attack Training}

In the zero-knowledge scenario, the attacker has no access to the victim classifier that they wish to attack, nor do they know its architecture.  This differs from the black box scenario in which the attacker can probe the victim classifier through an API, then observe the victim classifier's input-output relationship.  Instead, the attacker must rely entirely on the transferability of their attack to fool the victim CNN.

To achieve transferability, we propose adversarially training against an ensemble of forensic classifiers created by the attacker. 
%
Here, the classification loss $\mathcal{L}_c$ is formulated as the weights sum of individual classification loss pertaining to each CNN detector in the ensemble, 
\vspace{-0.5em}
\begin{equation}
\mathcal{L}_c= \sum_{s=1}^{S} \beta^{(s)} \mathcal{L}_c^{(s)}
\end{equation}
where $S$ is the number of CNN detectors in the ensemble, $ \mathcal{L}_c^{(s)}$ corresponds to individual classification loss of the $s^{th}$ CNN detector calculated using Equation~\ref{eq: white-box},  $\beta^{(s)}$ corresponds to the weight of  $s^{th}$ individual classification loss. 

Each classifier in the ensemble learns to partition the forensic feature space into separate regions for real and {\gi}s.  By defining the classifier loss in this fashion,  we incentivize the \ag to synthesize forensic features that lie in the intersection of these regions.  
If a diverse set of classifiers are used to form the ensemble, this intersection will likely lie inside the decision region that other classifiers associate with real images. 
 
We note that this approach differs from adversarially training against an ensemble classifier.  An ensemble classifier fuses the decisions of several weak classifiers to form an accurate representation of the ideal classification boundary separating real from {\gi}s.  We wish to avoid generating features in regions near the ideal decision boundary, since many different classifiers will likely make different decision in this region.  By synthesizing features that \textit{all} classifiers in our ensemble agree are real, we move away from the ambiguous region near the ideal decision boundary and further into the space that likely corresponds to real images.  








 


==> sections/proposed_v4_icpr.tex <==
% proposed
\section{Proposed Attack}

\subsection{Overivew}

Our attack is designed to modify a \gi $I$ so that a forensic CNN will instead classify it as a `real' image.  
This forensic CNN is alternately referred to as the victim classifier,  and is trained to differentiate between real and {\gi}s.

Our attack operates by passing the  \gi 
through a pre-trained \ag $G$ in order to falsify its forensic traces.  The \ag  is designed to remove forensic traces associated with {\gi}s and synthesize traces associated with `real' images.  
%
%As a result, a victim classifier, i.e. a forensic classifier that will be fooled by this attack, will misclassify the attacked GAN-generated image as a real one.
As a result, a victim classifier will  classify 
the attacked \gi $G(I)$ as a real one.
%
Furthermore, the \ag designed to make no changes to the image's contents and to introduce no visually perceptible distortions into the attacked image.  This will prevent a human from visually identifying that an image was attacked.  


The \ag in our attack learns to synthesize `real' forensic traces through adversarial training.   %The \ag 
It is trained as part of a GAN in which the discriminator is replaced by a forensic classifier (or set of classifiers) that has been pre-trained to learn the distribution of forensic features associated with real and {\gi}s.  

Different  strategies are used to train the \ag depending on whether the attack is launched in a white-box or zero-knowledge scenario. 
In the white-box scenario, our attack aims to synthesize forensic features with the distribution learned by the victim classifier, even if they deviate from the ideal feature distribution of real images.
%distribution of features associated with real images.
%
In the zero-knowledge scenario,  our attack aims to learn the  distribution of forensic features of real images.  However it avoids synthesizing features in regions where different classifiers may %use different decision boundaries.  
make different decisions.  
Instead,  it aims to synthesize features that any classifier will likely associate with a real image. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%   Below Removed To Save Space    %
%                                                     %
\begin{comment}
We  note that once our \ag is trained, our attack can be launched against any image without retraining.  Furthermore, since our attack is based on a convolutional generator, we can attack images of any size without the need to modify our generator or attack structure.  This differs from adversarial example generation techniques, which iteratively learn unique perturbations for each image that are the same size as the victim classifier's input.
\end{comment}
%                                                     %
%   Above Removed To Save Space   %
%                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%   Below Removed To Save Space    %
%                                                     %
\begin{comment}
\subsection{Difference From Adversarial Examples}
\input{sections/difference_from_adv_examples_v2}
\end{comment}
%                                                     %
%   Above Removed To Save Space   %
%                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{ Proposed Anti-Forensic Generator}
The proposed anti-forensic generator consists of a sequence of convolutional layers followed by ReLU activations~\cite{ReLU} shown in Figure~\ref{fig: generator}.   The first three convolutional layers use  64 filters,  the middle three convolutional layers use 128 filters,  and the final convolutional layer uses three filters to reduce the 128 feature maps to a three color channel image.  The output of the generator is the summation of the  input of the generator and the output of the last activated convolutional layer.  The skip connection is designed to give the generator  a better initialization for producing  high visual quality attacked images.
All convolutional layers use $3\times 3$ filter with stride 1.  The small filter size allows the generator to synthesize forensic traces in small areas.  We avoid using any pooling layers  to ensure that the output of the generator is of the same size as the input of the generator.  Therefore,  the proposed anti-forensic generator can be applied to images of arbitrary sizes,  and does not need to be trained for images of different sizes individually.   This characteristic  makes the deployment of the proposed  anti-forensic generator efficient and quick.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%   Below Removed To Save Space    %
%                                                     %
\begin{comment}
We note that our proposed generator is intentionally lightweight.  This allows it to be  trained using widely available commercial GPUs.  This also enables it to be quickly deployed at attack time.  
\end{comment}
%                                                     %
%   Above Removed To Save Space   %
%                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}[!t]
\centering
\includegraphics[width=0.45\textwidth]{figures/generator.pdf}
\caption{Architecture of the proposed anti-forensic generator.}
\label{fig: generator}
\end{figure}


%\subsection{Loss Function of the Adversarial Generator}
\subsection{Anti-Forensic Generator Training}

When adversarially training the \ag~$G$, we  formulate  a loss function 
%The loss function of the \ag is 
to ensure that a attacked image can both fool a victim classifier and maintain high visual quality.  
This  loss function $\mathcal{L}_{G}$ consists of the weighted sum of two terms: the perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$,  
\vspace{-0.5em}
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is used to balance the trade-off between the visual quality and performance of the attack. 


%%%%%%
%
\begin{comment}
The loss function of the adversarial generator is formulated to ensure the generated adversarial images both can fool forensic CNN detectors and maintain high visual quality.   The  loss function $\mathcal{L}_{G}$ is formulated as the weighted sum of perceptual loss $\mathcal{L}_{p}$ and classification loss $\mathcal{L}_{c}$ ,
\begin{equation}
\label{eq:g_loss}
\mathcal{L}_G=\alpha\mathcal{L}_p + \mathcal{L}_c,
\end{equation}
where $\alpha$ is the weight to balance the visual quality and performance of the attack. 
\end{comment}
%
%%%%%%%


%\underline{Perception loss} 
\subhead{Perceptual Loss} This term is used to minimize distortions introduced by the \ag and control the visual quality of the attacked image.  We define this term as  the mean absolute difference between the \gi $I$ (i.e the input of the generator ) and the attacked image produced by the generator $G(I)$, such that
\begin{equation}
\mathcal{L}_p = \,\tfrac{1}{N} \|I-G(I) \|_1,
\label{eq: perceptual_loss]}
\end{equation}
where $N$ is the number of pixels in $I$ and $G(I) $
  

\begin{comment}
is to ensure the visual quality of the generated images produces by the adversarial generator.  It is calcualted as the mean absolute different between the GAN-generated image $I$ (i.e input of the generator ) and the adversarial images produced by the attack,  
\begin{equation}
\mathcal{L}_p =\frac{1}{w\times h}\sum_{\ell=1}^{3}\sum_{i=1}^{w}\sum_{j=1}^{h}\mid I_{i,j}-G(I)_{i,j}\mid,
\label{eq: perceptual_loss]}
\end{equation}
where $G(\cdot)$ represents the adversarial generator,  and subscripts $i, j$ represent the pixel's coordinates.
\end{comment}


%\underline{Classification loss} 
\subhead{Classification Loss} This term is used to measure if  the  attacked images produced by the anti-forensic generator can fool the CNN detector used for training.  It allows the generator to learn forensic traces learned by the CNN detector.  The classification loss is provided by the victim  classifier for white-box attacks,   and  is provided by an ensemble of classifiers chosen by the attacker for zero-knowledge attacks.

%For white-box attacks,  the classification loss is provided by the victim  classifier.   For zero-knowledge attacks,   the classification loss is provided by an ensemble of classifiers chosen by the attacker. 

\begin{comment}
For a single CNN detector $C_s(\cdot)$ under attack,  the classification loss $\mathcal{L}_{c}^{(s)}$ is calculated as the softmax cross-entropy between the output of the CNN and the real class. 
\begin{equation}
\mathcal{L}_{c}^{(s)}=-\sum_{k=1}^{2} t_k \log\left(C_s(G(I))_k\right),
\label{eq: classification_loss}
\end{equation}
where $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ at the location of the unaltered class and $0$'s elsewhere. 
For the white-box attack,   the CNN detector is used for training the adversarial generator directly,  $\mathcal{L}_c=\mathcal{L}_c^{(s)}$.  For transferability in the zero-knowledge scenario,  t
\end{comment}

\subsection{White-Box Attack Training}

In the white-box scenario, the attacker has direct access to the forensic CNN under attack.  As a result, the \ag can be directly trained against the victim classifier.  In this case,  we define the classification
loss $\mathcal{L}_c$ as the softmax cross-entropy between the CNN detector's  output of attacked images and the real class.  Specifically,
\begin{equation}
	\mathcal{L}_c =-\sum_{k=1}^{2} t_k \log\left(C(G(I))_k\right),
	\label{eq: white-box}
\end{equation}
where $C(\cdot)$ is the victim classifier and  $t_k$ is the $k^{th}$ entry of ideal softmax vector with  a $1$ for the real class and a $0$ for the fake class.  
%
Defining the classification loss in this manner incentivizes the \ag to learn the victim classifier's model of forensic features from real images.  %that correspond to real images.









\subsection{Zero-Knowledge Attack Training}

In the zero-knowledge scenario, the attacker has no access to the victim classifier that they wish to attack, nor do they know its architecture.  This differs from the black box scenario in which the attacker can probe the victim classifier through an API, then observe the victim classifier's input-output relationship.  Instead, the attacker must rely entirely on the transferability of their attack to fool the victim CNN.

To achieve transferability, we propose adversarially training against an ensemble of forensic classifiers created by the attacker. 
%
Here, the classification loss $\mathcal{L}_c$ is formulated as the weights sum of individual classification loss pertaining to each CNN detector in the ensemble, 
\vspace{-0.5em}
\begin{equation}
\mathcal{L}_c= \sum_{s=1}^{S} \beta^{(s)} \mathcal{L}_c^{(s)}
\end{equation}
where $S$ is the number of CNN detectors in the ensemble, $ \mathcal{L}_c^{(s)}$ corresponds to individual classification loss of the $s^{th}$ CNN detector calculated using Equation~\ref{eq: white-box},  $\beta^{(s)}$ corresponds to the weight of  $s^{th}$ individual classification loss. 

Each classifier in the ensemble learns to partition the forensic feature space into separate regions for real and {\gi}s.  By defining the classifier loss in this fashion,  we incentivize the \ag to synthesize forensic features that lie in the intersection of these regions.  
If a diverse set of classifiers are used to form the ensemble, this intersection will likely lie inside the decision region that other classifiers associate with real images. 
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%   Below Removed To Save Space    %
%                                                     %
\begin{comment}

We note that this approach differs from adversarially training against an ensemble classifier.  An ensemble classifier fuses the decisions of several weak classifiers to form an accurate representation of the ideal classification boundary separating real from {\gi}s.  We wish to avoid generating features in regions near the ideal decision boundary, since many different classifiers will likely make different decision in this region.  By synthesizing features that \textit{all} classifiers in our ensemble agree are real, we move away from the ambiguous region near the ideal decision boundary and further into the space that likely corresponds to real images.  

\end{comment}
%                                                     %
%   Above Removed To Save Space   %
%                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%







 


==> sections/results.tex <==
%results and discussion
\section{Results and Discussions}
In this section,  we present and discuss the results achieved on the  human face dataset and the object dataset in the white-box scenario and the zero-knowledge scenario. 
\subsection{Results for White-Box Attack}

\input{sections/whitebox_results}

\subsection{Results for Zero-Knowledge Attack}

\input{sections/zero_results}


%\subsection{Sychronizing of Blocking}
\subsection{Invariance to Detection Block Alignment}
%When confronted with large {\gi}s, synthetic image detection CNNs typically analyze a small block of the image.  Many existing adversarial attacks assume prior knowledge of  location the block that the detector will analyze.

When confronted with large {\gi}s, synthetic image detection CNNs typically analyze 
either one or several smaller blocks of the image.
% a small block of the image. 
Many existing adversarial attacks either assume that all images are the same size as the victim classifier's input, or that the location of the block (or blocks) analyzed by the victim classifier is know to the attacker.  
%
By contrast, our proposed attack requires no advanced knowledge of the block or blocks that the victim classifier will analyze.  Since our attack is deployed via a fully convolution generator, it can be used to attack an entire image of arbitrary size.  Any  block analyzed by the victim CNN will contain falsified forensic traces.  

We demonstrated that our proposed attack is agnostic to blocking synchronization with the victim CNN by evaluating the proposed attack on large scale images (i.e bigger than the input size of the victim classifier).  Specifically, this can be seen by examining our attacks ASR 
using  StyleGAN and StyleGAN2 generated images of  human faces as shown in Table~\ref{tab: whiteboxface},  since they are of size $1024\times 1024$.   
Our \ag was trained using $256\times 256$ in the attacker's training set, then deployed on the full sized $1024\times 1024$ images in the evaluation set.  The victim CNNs analyzed these images by randomly cropping a $256\times 256$ image block for analysis.  
The high attack success rates achieved on attacking  StyleGAN and StyleGAN2 generated images of  human faces demonstrates that a randomly selected image patch from the attacked image can still fool the CNN detectors.  





%Since the detection algorithms using CNNs  usually operate on predicting image patches rather than the full-size image,  many existing adversarial attacks requires the prior knowledge of blocking grids.  However,  our proposed attack  requires no prior knowledge of blocking grids.   It means that once the generator was trained,  it can be applied directly to any full-size image,  and any patches from the attacked image  should be able to fool the CNN detectors. 

%We demonstrated that our proposed attack is agnostic to blocking synchronization by evaluating the proposed attack on large scale images (i.e bigger than the input size of the CNN detectors).  In this paper,  we demonstrated the results using  StyleGAN and StyleGAN2 generated images of  human faces,  because they are of resolution $1024\times 1024$.   To evaluate the attacked images produced from large scale images,  we first applied trained anti-forensic  generator to the $1024\times 1024$ full-size images at once,   then randomly cropped a $256\times 256$ image window for CNN detection.  The high attack success rates achieved on attacking  StyleGAN and StyleGAN2 generated images of  human faces demonstrates that a randomly selected image patch from the attacked image can still fool the CNN detectors.  




==> sections/results_v2_icpr.tex <==
%results and discussion
\section{Results and Discussions}
In this section,  we present and discuss the results achieved on the  human face dataset and the object dataset in the white-box scenario and the zero-knowledge scenario. 
\subsection{Results for White-Box Attack}

\input{sections/whitebox_results_v3_icpr}

\subsection{Results for Zero-Knowledge Attack}

\input{sections/zero_results_v1_icpr}



%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                     %
%   Below Removed To Save Space    %
%                                                     %
\begin{comment}
%\subsection{Sychronizing of Blocking}
\subsection{Invariance to Detection Block Alignment}
%When confronted with large {\gi}s, synthetic image detection CNNs typically analyze a small block of the image.  Many existing adversarial attacks assume prior knowledge of  location the block that the detector will analyze.

When confronted with large {\gi}s, synthetic image detection CNNs typically analyze 
either one or several smaller blocks of the image.
% a small block of the image. 
Many existing adversarial attacks either assume that all images are the same size as the victim classifier's input, or that the location of the block (or blocks) analyzed by the victim classifier is know to the attacker.  
%
By contrast, our proposed attack requires no advanced knowledge of the block or blocks that the victim classifier will analyze.  Since our attack is deployed via a fully convolution generator, it can be used to attack an entire image of arbitrary size.  Any  block analyzed by the victim CNN will contain falsified forensic traces.  

We demonstrated that our proposed attack is agnostic to blocking synchronization with the victim CNN by evaluating the proposed attack on large scale images (i.e bigger than the input size of the victim classifier).  Specifically, this can be seen by examining our attacks ASR 
using  StyleGAN and StyleGAN2 generated images of  human faces as shown in Table~\ref{tab: whiteboxface},  since they are of size $1024\times 1024$.   
Our \ag was trained using $256\times 256$ in the attacker's training set, then deployed on the full sized $1024\times 1024$ images in the evaluation set.  The victim CNNs analyzed these images by randomly cropping a $256\times 256$ image block for analysis.  
The high attack success rates achieved on attacking  StyleGAN and StyleGAN2 generated images of  human faces demonstrates that a randomly selected image patch from the attacked image can still fool the CNN detectors.  
\end{comment}
%                                                     %
%   Above Removed To Save Space   %
%                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> sections/unaligned.tex <==
%Unaligned JPEG

\begin{table}
\centering
\caption{random crop }
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{|l|cc||cc|}
\hline
\multicolumn{1}{|c}{}&\multicolumn{2}{|c||}{\textbf{White-Box}}&\multicolumn{2}{c|}{\textbf{Zero Knowledge}}\\
\hline

\textbf{Models}& \textbf{StyleGAN} &\textbf{StyleGAN2}& \textbf{StyleGAN} &\textbf{StyleGAN2}\\
\textbf{MISLNet}&&&&\\
\textbf{PHNet}&&&&\\
\textbf{SRNet} &0.9180& 0.9070& & \\
\textbf{Stega CNN}&&&&\\
\textbf{Tuama CNN}&&&&\\
\textbf{ResNet50}&&&&\\
\textbf{DenseNet}&&&&\\
\textbf{Xception}&&&&\\
\hline
\end{tabular}}
\end{table}

==> sections/whitebox_results.tex <==
%white box results 
\begin{comment}
\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of human faces in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|cccc||cc|}
\hline
\multicolumn{7}{|c|}{\textbf{Proposed Adversarial Generator}}\\\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} &1.0000 &1.0000 &1.0000 &\textbf{1.0000}& 45.52&0.9875\\
\textbf{ResNet-50} &  0.7590 & 0.8770& 0.8010 &\textbf{0.8123}&35.97 &0.9578\\
\textbf{DenseNet}&0.9385 & 0.9770& 0.9970&\textbf{0.9708} &54.28&0.9997\\
\textbf{MISLNet}& 0.9965  & 0.9905 &0.9950&\textbf{0.9940}&51.28 &0.9925\\
\textbf{PHNet} &  1.0000&0.8497 &0.9985& \textbf{0.9494}&41.85&0.9753\\
\textbf{SRNet} &  0.8080&0.8855 &0.9480&\textbf{0.8805}&50.97 &0.9922\\
\textbf{ImageCNN} &  0.9854&0.9935 & 0.8505&\textbf{0.9431}&53.64 &0.9928\\
\textbf{CamID CNN} &0.9285 &0.9120& 0.9870& \textbf{0.9425}& 58.10&0.9988\\
\textbf{Avg.}&\textbf{0.9270}&\textbf{0.9357}&\textbf{0.9471}&\textbf{0.9366}&\textbf{48.95}&\textbf{0.9871}\\
\hline

\multicolumn{7}{|c|}{\textbf{Residual Generator~\cite{residualgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception}& 0.9820&0.9940 &0.9770& 0.9843&29.01 &0.9498\\
\textbf{ResNet-50}& 0.1435 & 0.6010&0.5375&0.4273& 28.82&0.9448\\
\textbf{DenseNet}& 0.9915& 0.9955&0.9940 &0.9937& 29.72&0.9515\\
\textbf{MISLNet}&  0.9605&  0.9970&0.9880 & 0.9818&29.82& 0.9440\\
\textbf{PHNet} & 0.9665&0.9470 &0.9915 &0.9683 &30.21 &0.9556\\
\textbf{SRNet} &0.9605 & 0.9885& 0.9770&0.9753&29.46&0.9474\\
\textbf{Image CNN} & 1.0000&0.0000 & 1.0000&0.6667&29.21 &0.9531\\
\textbf{CamID CNN}& 0.9955& 0.9995&0.9990& 0.9980&28.89&0.9536\\
\textbf{Avg.} &0.8750&0.8150&0.9330&0.8744&29.39&0.9500\\

\hline
\multicolumn{7}{|c|}{\textbf{MISLGAN Generator~\cite{mislgan}}}\\
\hline
\textbf{CNNs}& \textbf{StarGAN-v2} & \textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{M\textunderscore SSIM}\\
\textbf{Xception} & 1.0000& 0.0005& 1.0000&0.6668& 32.24&0.9598\\
\textbf{ResNet-50}& 0.4235&0.8115 & 0.7465&0.6605&34.64 &0.9630\\
\textbf{DenseNet}& 0.9995&1.0000 &0.9995 &0.9997 &35.11&0.9755\\
\textbf{MISLNet}& 0.9515 &  0.9965&0.9899 &0.9793 &34.50&0.9660 \\
\textbf{PHNet} & 0.9925& 0.9995 & 0.9985&0.9968&34.84 &0.9648\\
\textbf{SRNet} & 0.8915 & 0.9735&0.9635 &0.9428&33.09 &0.9550\\
\textbf{Image CNN} &0.7975 & 0.7980& 0.8205 &0.8053&34.36&0.9657\\
\textbf{CamID CNN}& 0.5410&0.3540 & 0.3720&0.4223& 33.30&0.9669\\
\textbf{Avg.} &0.8246&0.7417&0.8613&0.8092&34.01&0.9646\\
\hline
\end{tabular}}
\label{tab: whiteboxface}
\end{table}

\begin{table}[!t]
\centering
%\caption{Evaluation of attacks against victim CNNs for detecting GAN-generated images of objects in the white-box scenario. }
\caption{Attack success rates and image quality achieved for white-box attacks on the Object Dataset.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|ccccccc||cc|}
\hline
\multicolumn{10}{|c|}{\textbf{Proposed Adversarial Generator}}\\
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.}&\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM}\\
\textbf{Xception} &0.9880 &0.9871 &0.9995 & 1.0000 & 0.9975& 0.9992&\textbf{0.9952}&52.59&0.9972 \\
\textbf{ResNet-50} &0.9174 &0.8720 & 0.9910& 0.9971& 0.9520&0.9848 &\textbf{0.9524}&55.41&0.9973 \\
\textbf{DenseNet}  & 0.8583&0.8432 &0.9457 & 0.9474&0.9350 & 0.9402&\textbf{0.9116}&50.22&0.9893\\
\textbf{MISLNet} & 0.9437& 0.6409& 0.9893& 0.9954&0.9930&0.9994&\textbf{0.9270}&50.97&0.9925 \\
\textbf{PHNet}  & 0.9645 &0.9477 &0.9834 & 0.9985& 0.9890& 0.9978& \textbf{0.9802}&51.99&0.9613\\
\textbf{SRNet} & 0.7980 & 0.5758 & 0.9577& 0.9959& 0.7600& 0.8846&\textbf{0.8287}&56.41&0.9940\\
\textbf{Image CNN} &0.6890 & 0.6644 & 0.9341&0.9772  &0.8540 & 0.7152&\textbf{0.8057}&55.32&0.9981\\
\textbf{CamID CNN} & 0.8650 &0.8470 & 0.9694&0.9622 & 0.9445& 0.9946&\textbf{0.9305}&52.77 &0.9970\\
\textbf{Avg.} &\textbf{0.8780}&\textbf{0.7973}&\textbf{0.9713}&\textbf{0.9842}&\textbf{0.9281}&\textbf{0.9395}&\textbf{0.9164}&\textbf{53.21}&\textbf{0.9908}\\
\hline
\multicolumn{10}{|c|}{\textbf{Residual Generator~\cite{residualgan}}}\\
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.} &\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM} \\
\textbf{Xception} &0.9927 &0.9954 &0.9983 & 0.9936 & 0.9975 & 1.0000 &0.9963&39.73&0.9612 \\
\textbf{ResNet-50} &0.9197    &0.9447 & 0.9376& 0.9588 & 0.9490 & 0.9670&0.9461&38.51&0.9728\\
\textbf{DenseNet}  &0.9582 & 0.9242&0.9677 & 0.9724&0.9585 & 0.9322&0.9522&37.52&0.9543\\
\textbf{MISLNet} & 0.7800 & 0.6068& 0.7952& 0.9644& 0.8910 & 0.9934&0.8353&40.49&0.9875 \\
\textbf{PHNet}  & 0.9287 &0.9758 &0.9405 & 0.9766 & 0.9745& 0.9916& 0.9646&40.22&0.9719\\
\textbf{SRNet} & 0.7215&0.6485 &0.8590  &0.9658  &0.8180 &0.9110 &0.8206&37.36&0.9649\\
\textbf{Image CNN} &0.6580 &  0.6114 & 0.7811 & 0.9543 &0.5905 & 0.2096& 0.6342&38.66&0.9679\\
\textbf{CamID CNN} & 0.6207 &0.6121 & 0.8789&0.9669 &0.8860 & 0.8590&0.8039&39.02 &0.9736\\
\textbf{Avg.} &0.8224&0.7899&0.8949&0.9691&0.8831&0.8580&0.8695&38.94&0.9693\\
\hline
\multicolumn{10}{|c|}{\textbf{MISLGAN Generator~\cite{mislgan}}}\\
\hline
\textbf{CNNs}&\textbf{ProGAN}&\textbf{CycleGAN} &\textbf{StyleGAN}&\textbf{StyleGAN2}&\textbf{BigGAN}&\textbf{GauGAN}&\textbf{Avg.} &\textbf{M\textunderscore PSNR}&\textbf{ M\textunderscore SSIM} \\
\textbf{Xception} &0.9405 & 0.9477& 0.9666&  0.9783&0.9155 & 0.9414&0.9483&32.09&0.9651 \\
\textbf{ResNet-50} & 0.9117&0.8955 & 0.9025& 0.7645& 0.9614& 0.8720&0.8846& 31.50&0.9547\\
\textbf{DenseNet}  &0.9687 & 0.9227 & 0.9674& 0.9772& 0.9300& 0.9432&0.9515&31.22&0.8470\\
\textbf{MISLNet} &0.9905 & 0.9905 &0.9915 &0.9880 &0.9910  &0.9955 &0.9912&31.75& 0.9602\\
\textbf{PHNet}  & 0.8200&0.8465 & 0.8215&0.8250 &0.8305  &0.8405 & 0.8307&31.00&0.9495 \\
\textbf{SRNet} & 0.9230 & 0.8114 & 0.9719& 0.9979&  0.9495&0.9896 & 0.9406&31.68& 0.9689\\
\textbf{Image CNN} & 0.7333& 0.7205  & 0.8879& 0.9866 & 0.8000& 0.7368&0.8109 & 33.43&0.8750\\
\textbf{CamID CNN} &  0.6925& 0.6636& 0.7821& 0.9417& 0.6995&0.7618 &0.7569& 31.37&0.9120\\
\textbf{Avg.} &0.8725&0.8498&0.9114&0.9324&0.8847&0.8851&0.8893&31.76&0.9291\\
\hline
\end{tabular}}
\label{tab: whiteboxobject}
\end{table}
\end{comment}

\begin{table}
\centering
\caption{Attack success rates and image quality achieved for white-box attacks on the Human Face Dataset. }
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
CNNs & CW,  mPSNR & FGSM,  mPSNR & PGD,  mPSNR & Proposed,  mPSNR\\
Xception & & & & \\
\end{tabular}|
\end{table}


Table~\ref{tab: whiteboxface} shows the  performance our attack achieved on the human face dataset,  and Table~\ref{tab: whiteboxobject} shows performance of our attack on the object  dataset.  Attack success rates, defined as the percentage of attacked images classified as `real' images,  are shown to the left of the double bar, while image quality measures (mean PSNR and mean SSIM) are shown to the right.

%Attack success rates achieved against the victim CNN detectors are shown in the left  sections of the tables.   Mean PSNR and mean SSIM are shown in the right sections of the tables.

%\subhead{Attack Success Rates on the Human Face Dataset}
\subhead{Human Face Dataset Attack Success Rates}
Each entry in the left section of Table~\ref{tab: whiteboxface}  corresponds to the attack success rate against a particular victim CNN detector.  On average,  our proposed attack achieved $0.9366$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of human faces.  Particularly,   the proposed attack achieved above $0.90$ average attack success rate associated with each GAN method.  This means the proposed attack can successfully falsify forensic traces left by StyleGAN,  StyleGAN2, and StarGAN-v2.  Additionally,  the average attack success rates associated with each CNN detector were mostly above $0.94$.  It means that the proposed attack can  fool each victim CNN detector strongly.  

%\subhead{Attack Success Rates on the Object Dataset}
\subhead{Object Dataset Attack Success Rates}
Each entry in the left section of Table~\ref{tab: whiteboxobject} corresponds to  the  attack success rate  achieved on the object dataset against a particular victim CNN detector.  On average,  the proposed attack achieved $0.9164$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of objects.  The average attack success rates associated with each GAN method  are mostly above $0.9000$.  The results showed  that the proposed attack can falsify forensic traces left by a variety of GAN methods. 
The average attack success rates associated with each  CNN detector are mostly above $0.9000$.  These results showed the proposed attack can successfully fool individual victim CNN detector strongly. 
We note that for attacks on the object dataset,  the proposed attacks were trained only using ProGAN generated images.  However,  the proposed attack can still fool the CNN detectors when applying the attack on generated images produced by other GAN methods.  It means that the proposed attack can remove  forensic traces left by unseen GAN methods. 

\begin{figure}[!t]
\includegraphics[width=0.48\textwidth]{figures/object_demo}
\caption{Attacked images produced by our white-box attack. }
%Attacked images produced by the proposed anti-forensic generator trained on the object dataset.  The  anti-forensic generator used to create the demo attacked  images was trained to attack ResNet-50 in the white-box scenario. }
\label{fig: object_demo}
\end{figure}

\subhead{Visual Quality} The right sections of Table~\ref{tab: whiteboxface} and Table~\ref{tab: whiteboxobject} show the evaluation of the image quality of attacked images produced by the proposed attack.  On the human face dataset,  the average mean PSNR is $48.95$ and the average mean SSIM $0.9871$.  On the object dataset,  the average mean PSNR is $53.21$ and the average mean SSIM $0.9908$.   The results mean the attacked images produced by our proposed attack can maintain very high visual quality. 

We present attacked images produced by the proposed attack in Figure~\ref{fig: object_demo}.   These attacked images were created using the anti-forensic generator trained against ResNet-50.  Visually comparing the GAN-generated images to the attacked images, we can see that there is no visible difference between the two. This demonstrates that our attack will not leave behind visual cues and it will not alter the content of the attacked image in an undesirable manner.

\subhead{Comparing with Other Generators} We compared the performance of the proposed anti-forensic generator with two previous work~\cite{residualgan,mislgan} that also used GAN-based generators to falsify forensic traces of images.  

In terms of attack success rates,  Table ~\ref{tab: whiteboxface} shows that  on the human face dataset,  our proposed generator achieved $6\%$ higher on average than the residual generator~\cite{residualgan},  and $12\%$ higher than the MISLGAN generator.  Table ~\ref{tab: whiteboxobject} shows that  on the object dataset,  our proposed generator achieved $4.5 \%$ higher on average  than the residual generator~\cite{residualgan},  and $12\%$ higher than the MISLGAN generator.  

In terms of image quality,  on both datasets our proposed attack dramatically outperforms the other two generators.  On the human face dataset,  the proposed generator achieved $20$ dB higher mean PSNR than the residual generator and $15$ dB higher mean PSNR than the MISLGAN generator,  $3\%$ higher mean SSIM than the residual generator and $2.5\%$ higher mean SSIM than the MISLGAN generator.  On the object dataset,  the proposed generator achieved $14$ dB higher mean PSNR than the residual generator and $21$ dB higher mean PSNR than the MISLGAN generator,  $2\%$ higher mean SSIM than the residual generator and $6\%$ higher mean SSIM than the MISLGAN generator.

To summarize,  in the white-box scenario,  we demonstrated that our proposed attack can successfully fool victim CNN detectors on both the human face dataset and the object dataset. 
The attacked images produced by our attack have high visual quality.  We also demonstrated that our proposed attack outperformed previous works.








==> sections/whitebox_results_v2_icpr.tex <==
%white box results 

% Old/Debug
%\input{sections/GenArchComp-Face.tex}
%\input{sections/GenArchComp-Face-Full.tex}


\def\tablesize{0.85}
\def\tablesizetwo{1.0}

%\input{sections/WhiteBox-Face-Full.tex}
%\input{sections/WhiteBox-Object-Full.tex}
\input{sections/WhiteboxBoth.tex}
%\input{sections/Zero-Face-Full.tex}
%\input{sections/Zero-Object-Full.tex}

\input{sections/ZeroBoth.tex}

Table~\ref{tab: whiteboxface} shows the  performances of attacks achieved on both datasets.   Attack success rates, defined as the percentage of attacked images classified as `real' images,  mean of PSNRs measures the image quality of attacked images.  


%Attack success rates achieved against the victim CNN detectors are shown in the left  sections of the tables.   Mean PSNR and mean SSIM are shown in the right sections of the tables.

\subhead{Human Face Dataset Attack Success Rates}
Each row under the column ``Proposed"of Table~\ref{tab: whiteboxface}  shows the mean attack success  rate and mean PSNR of our proposed attack against a particular victim CNN detector. 
%Each entry in the left section of Table~\ref{tab: whiteboxface}  corresponds to the attack success rate against a particular victim CNN detector.  
On average,  our proposed attack achieved $0.9366$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of human faces.  %Particularly,   the proposed attack achieved above $0.90$ average attack success rate associated with each GAN method.  
This means the proposed attack can successfully falsify forensic traces left by StyleGAN,  StyleGAN2, and StarGAN-v2.  Additionally,   the mean attack success rates associated with each CNN detector were mostly above $0.94$.  It means that the proposed attack can  fool each victim CNN detector strongly.  

\subhead{Object Dataset Attack Success Rates}
Each row under the column proposed of Table~\ref{tab: whiteboxobject}  shows the mean attack success rate and mean PSNR of our proposed attack against a particular victim CNN detector. 
On average,  our proposed attack achieved $0.9164$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of objects.  The results showed  that the proposed attack can falsify forensic traces left by a variety of GAN methods. 
The mean  attack success rates associated with each  CNN detector are mostly above $0.90$.  These results showed the proposed attack can successfully fool each  victim CNN detector strongly. 
We note that for attacks on the object dataset,  the proposed attacks were trained only using ProGAN generated images.  However,  the proposed attack can still fool the CNN detectors when applying the attack on generated images produced by other GAN methods.  It means that the proposed attack can remove  forensic traces left by unseen GAN methods. 

\begin{figure}[!t]
\includegraphics[width=0.48\textwidth]{figures/object_demo}
\caption{Attacked images produced by the proposed white-box attack. }
\label{fig: object_demo}
\end{figure}

\subhead{Visual Quality} The average mean PSNR  is $48.95$dB  for the human face dataset and $53.21$dB for the object dataset.  It  means that  the attacked images produced by our proposed attack can maintain very high visual quality. 

%The right sections of Table~\ref{tab: whiteboxface} and Table~\ref{tab: whiteboxobject} show the evaluation of the image quality of attacked images produced by the proposed attack.  On the human face dataset,  the average mean PSNR  and the average mean SSIM $0.9871$.  On the object dataset,  the average mean PSNR is  and the average mean SSIM $0.9908$.  
We present attacked images  produced  by the proposed attack in Figure~\ref{fig: object_demo}.   These attacked images were created  using the anti-forensic generator trained against ResNet-50.  Visually comparing the GAN-generated images to the attacked images,  there is no visible difference between the two versions. This demonstrates that our proposed attack will not leave behind visual cues,  and it will not alter the contents of attacked images in an undesirable manner.

\subhead{Comparing with Other Generators} Previous research also used GAN-based attack to remove forensic traces left by manipulation operation,  and falsify camera model information.    Therefore,  we compared the performance of the proposed anti-forensic generator with two previous work~\cite{residualgan,mislgan}. 

In terms of attack success rates,  Table ~\ref{tab: whiteboxface} shows that  on the human face dataset,  our proposed generator achieved $6\%$ higher on average than the residual generator~\cite{residualgan},  and $12\%$ higher than the MISLGAN generator.  Table ~\ref{tab: whiteboxobject} shows that  on the object dataset,  our proposed generator achieved $4.5 \%$ higher on average  than the residual generator~\cite{residualgan},  and $12\%$ higher than the MISLGAN generator.  

In terms of image quality,  on both datasets our proposed attack significantly outperforms the other two generator architectures.  On the human face dataset,  the proposed generator achieved $20$dB higher mean PSNR than the residual generator and $15$dB higher mean PSNR than the MISLGAN generator.
%$3\%$ higher mean SSIM than the residual generator and $2.5\%$ higher mean SSIM than the MISLGAN generator.  
On the object dataset,  the proposed generator achieved $14$dB higher mean PSNR than the residual generator and $21$dB higher mean PSNR than the MISLGAN generator.
%$2\%$ higher mean SSIM than the residual generator and $6\%$ higher mean SSIM than the MISLGAN generator.

\subhead{Comparing with Adversarial Example Attacks} Adversarial example attacks are commonly used to fool CNN-based classifiers.  We compared our proposed attack with three most well-known adversarial example attacks,  CW attack~\cite{cw},  FGSM attack~\cite{fgsm} and PGD attack~\cite{pgd}.  We used the public available toolbox CleverHans~\cite{papernot2018cleverhans} to launch these attacks. 

To attack a image using adversarial example attacks,  the attacks need to be trained specifically on that image.   With a GTX 1080 Ti GPU,    attacking all  testing images  in one dataset using one adversarial attack will take over 10 hours.   To the best usage of time,   we randomly chose 260 images from the test set of each dataset to evaluate the performance of adversarial attacks. 

It is well-known that a stronger attack typically means more visible perturbations.  However,  unlike attacking CNNs for computer vision task,  performing attacks for anti-forensic purposes have a higher requirement for maintaining the visual quality,  since an image full of speckles can never pass human inspection.  As a result,  for a fair comparison,  we chose the parameters for each adversarial example attack such that the mean PSNRs of produced attacked images were on the same level as our proposed attack,  and then we compared the performances of adversarial example attacks with our proposed attack in terms of mean attack success rates.


On human face dataset,  Table~\ref{tab: whiteboxface} shows that on average  CW attack achieved  $ 0. 8982$ attack success rate,  FGSM attack achieved $ 0.5147$ attack success rate,  and PGD attack achieved $ 0.9286$ attack success rate,   comparing with the proposed attack that achieved $0.9366$ attack success rate.   It shows that when the attacked images have  similar visual quality,  our proposed attack outperforms the adversarial example attacks.  Additionally,  we noted that the  FGSM attack performed the worst among the three adversarial example attacks,  while PGD attacks performed the best with  the average attack success rate  close to ours.  However,   all three attacks had some difficulty in fooling ResNet-50,  while our proposed attack can uniformly fool all CNN detectors. 

On object dataset,  Table~\ref{tab: whiteboxface} shows that on average  CW attack achieved  $ 0. 7162$ attack success rate,  FGSM attack achieved $ 0.6319$ attack success rate,  and PGD attack achieved $ 0.7367$ attack success rate,   comparing with the proposed attack that achieved $0.9164$ attack success rate.  It again shows that our proposed attack outperforms the adversarial attacks. 


%To summarize,  in the white-box scenario,  we demonstrated that our proposed attack can successfully fool victim CNN detectors on both the human face dataset and the object dataset.  The attacked images produced by our attack have high visual quality.  We also demonstrated that our proposed attack outperformed other alternative attacks. 








==> sections/whitebox_results_v3_icpr.tex <==
%white box results 

% Old/Debug
%\input{sections/GenArchComp-Face.tex}
%\input{sections/GenArchComp-Face-Full.tex}


\def\tablesize{0.85}
\def\tablesizetwo{1.0}

%\input{sections/WhiteBox-Face-Full.tex}
%\input{sections/WhiteBox-Object-Full.tex}
\input{sections/WhiteboxBoth.tex}
%\input{sections/Zero-Face-Full.tex}
%\input{sections/Zero-Object-Full.tex}

\input{sections/ZeroBoth.tex}
Table~\rom{2} shows the  performances of attacks achieved on both datasets in white-box scenarios.   Attack success rates(ASRs), defined as the percentage of attacked images classified as `real' images,  mean of PSNRs measures the image quality of attacked images.  Each entry in the table corresponds to the mean attack success rates and mean PSNR  achieved by an attack when attacking a particular victim CNN detector.


%Attack success rates achieved against the victim CNN detectors are shown in the left  sections of the tables.   Mean PSNR and mean SSIM are shown in the right sections of the tables.

\subhead{Human Face Dataset Attack Success Rates}
The top half  of Table~\rom{2}  shows the performances of attacks using the human face dataset.
%Each entry in the left section of Table~\ref{tab: whiteboxface}  corresponds to the attack success rate against a particular victim CNN detector.  
On average,  our proposed attack achieved $0.9366$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of human faces.  %Particularly,   the proposed attack achieved above $0.90$ average attack success rate associated with each GAN method.  
This means the proposed attack can successfully falsify forensic traces left by StyleGAN,  StyleGAN2, and StarGAN-v2.  Additionally,   the mean attack success rates associated with each CNN detector were mostly above $0.94$.  It means that the proposed attack can  fool each victim CNN detector strongly.  

\subhead{Object Dataset Attack Success Rates}
The bottom half  of Table~\rom{2} shows the performances of attacks using the object dataset.
On average,  our proposed attack achieved $0.9164$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of objects.  The results showed  that the proposed attack can falsify forensic traces left by a variety of GAN methods. 
The mean  attack success rates associated with each  CNN detector are mostly above $0.90$.  These results showed the proposed attack can successfully fool each  victim CNN detector strongly. 
We note that for attacks on the object dataset,  the proposed attacks were trained only using ProGAN generated images.  However,  the proposed attack can still fool the CNN detectors when applying the attack on generated images produced by other GAN methods.  It means that the proposed attack can remove  forensic traces left by unseen GAN methods. 

\begin{figure}[!t]
\includegraphics[width=0.48\textwidth]{figures/object_demo}
\caption{Attacked images produced by the proposed white-box attack. }
\label{fig: object_demo}
\end{figure}

\subhead{Visual Quality} The average mean PSNR  is $48.95$dB  for the human face dataset and $53.21$dB for the object dataset.  It  means that  the attacked images produced by our proposed attack can maintain very high visual quality. 

%The right sections of Table~\ref{tab: whiteboxface} and Table~\ref{tab: whiteboxobject} show the evaluation of the image quality of attacked images produced by the proposed attack.  On the human face dataset,  the average mean PSNR  and the average mean SSIM $0.9871$.  On the object dataset,  the average mean PSNR is  and the average mean SSIM $0.9908$.  
We present attacked images  produced  by the proposed attack in Figure~\ref{fig: object_demo}.   These attacked images were created  using the anti-forensic generator trained against ResNet-50.  Visually comparing the GAN-generated images to the attacked images,  there is no visible difference between the two versions. This demonstrates that our proposed attack will not leave behind visual cues,  and it will not alter the contents of attacked images in an undesirable manner.

\subhead{Comparing with Other Generators} We compared the performance of the proposed anti-forensic generator with two previous work~\cite{residualgan,mislgan}. 

In terms of attack success rates,   on the human face dataset,  our proposed generator achieved $6\%$ higher on average than the residual generator~\cite{residualgan},  and $12\%$ higher than the MISLGAN generator.   On the object dataset,  our proposed generator achieved $4.5 \%$ higher on average  than the residual generator~\cite{residualgan},  and $12\%$ higher than the MISLGAN generator.  

In terms of image quality,  on both datasets our proposed attack significantly outperforms the other two generator architectures.  On the human face dataset,  the proposed generator achieved $20$dB higher mean PSNR than the residual generator and $15$dB higher mean PSNR than the MISLGAN generator.
%$3\%$ higher mean SSIM than the residual generator and $2.5\%$ higher mean SSIM than the MISLGAN generator.  
On the object dataset,  the proposed generator achieved $14$dB higher mean PSNR than the residual generator and $21$dB higher mean PSNR than the MISLGAN generator.
%$2\%$ higher mean SSIM than the residual generator and $6\%$ higher mean SSIM than the MISLGAN generator.

\subhead{Comparing with Adversarial Example Attacks} We also compared our proposed attack with three most well-known adversarial example attacks,  CW~\cite{cw},  FGSM~\cite{fgsm} and PGD~\cite{pgd}.  We used the public available toolbox CleverHans~\cite{papernot2018cleverhans} to launch these attacks. 

To attack a image using adversarial example attacks,  the attacks need to be trained specifically on that image.   With a GTX 1080 Ti GPU,    attacking all  testing images  in one dataset using one adversarial attack will take over 10 hours.   To the best usage of time,   we randomly chose 260 images from the test set of each dataset to evaluate the performance of adversarial attacks. 

It is well-known that a stronger attack typically means more visible perturbations.  However,  unlike attacking CNNs for computer vision task,  performing attacks for anti-forensic purposes have a higher requirement for maintaining the visual quality,  since an image full of speckles can never pass human inspection.  As a result,  for a fair comparison,  we chose the parameters for each adversarial example attack such that the mean PSNRs of produced attacked images were on the same level as our proposed attack,  and then we compared the performances of adversarial example attacks with our proposed attack in terms of mean attack success rates.


For the human face dataset,  on average  CW attack achieved  $ 0. 8982$ attack success rate,  FGSM attack achieved $ 0.5147$ attack success rate,  and PGD attack achieved $ 0.9286$ attack success rate,   while  the proposed attack that achieved $0.9366$ attack success rate.   These results show that when the attacked images have  similar visual quality,  our proposed attack outperforms the adversarial example attacks.  Additionally,  we noted that the  FGSM attack performed the worst among these adversarial example attacks,  while PGD attacks performed the best with  the average attack success rate close to ours.  However,   all three attacks had some difficulty in fooling ResNet-50,  while our proposed attack can uniformly fool all CNN detectors. 

For the object dataset,   on average  CW attack achieved  $ 0. 7162$ attack success rate,  FGSM attack achieved $ 0.6319$ attack success rate,  and PGD attack achieved $ 0.7367$ attack success rate,   while  the proposed attack that achieved $0.9164$ attack success rate.  These results again show that our proposed attack outperforms the adversarial attacks. 


%To summarize,  in the white-box scenario,  we demonstrated that our proposed attack can successfully fool victim CNN detectors on both the human face dataset and the object dataset.  The attacked images produced by our attack have high visual quality.  We also demonstrated that our proposed attack outperformed other alternative attacks. 








==> sections/zero_results.tex <==
%zero knowledge results

Table~\ref{tab: zeroface} shows the  performance our attack achieved on the human face dataset,  and Table~\ref{tab: zeroobject} shows performance of our attack on the object dataset.   


\subhead{Human Face Dataset Attack Success Rates} 
Each row under the column proposed of Table~\ref{tab: zeroface}  shows the mean attack success  rate and mean PSNR of our proposed attack against a particular victim CNN detector.  On average,  the proposed attack achieved $0. 7510$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of human faces.   While the average attack success rate decreased $15\%$ comparing with  the white-box scenario,   it was mainly because of low attack success rates against ResNet-50 and MISLNet.  We still achieved high attack success rates for the other six CNN detectors. 

\subhead{Object Dataset Attack Success Rates}
Each row under the column proposed of Table~\ref{tab: zeroobject}  shows the mean attack success  rate and mean PSNR of our proposed attack against a particular victim CNN detector.  On average,  the proposed attack achieved $0.7030$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of objects.  We note that the drop on the average attack success rate comparing to the white-box scenario was mainly caused by SRNet and MISLNet.  We still achieved high attack success rates for the  other six CNN detectors.  

\subhead{Interpretation of the Results}The attack success rates achieved on both datasets demonstrate that the proposed attack can  transfer to fool CNN detectors even when the attacker has zero-knowledge about the CNN detectors.  The results are important because it shows that our attack can be launched in a realistic scenario.  While the results are not perfect,  particularly in the attacks  against  ResNet-50 and MISLNet on the  human faces dataset and the attacks against MISLNet and SRNet on the object dataset,  the results still strongly show that the proposed attack can pose enough threat,  since it worked  great on the majority of the testing cases.  For example,  the attack success rates against Xception are uniformly high (over $0.90$) on both datasets.  
One possible explanation for the low attack success rates in some cases could be that  forensic traces learned by these victim CNN detectors are not located in the same feature space as the ensemble of CNN detectors used to train the attack.   However,  we think it may provide some insights for the investigators and researchers  developing  defense strategies against similar types of attack. 


\subhead{Visual Quality} 
The average mean PSNR  is $40.46$dB  for the human face dataset and $41.27$dB for the object dataset.  These results show that  the attacked images produced by our proposed attack can maintain very high visual quality. 
%The right sections of Table~\ref{tab: zeroface} and Table~\ref{tab: zeroobject} show the evaluation of the image quality of attacked images produced by the proposed attack.    On the human face dataset,  the average mean PSNR is $40.46$ and the average mean SSIM is $0.9682$.  On the object database,  the average mean PSNR is $41. 27$ and the average mean SSIM is $0.9456$.  

We present attacked images of human faces produced by the proposed attack  in Figure~\ref{fig: face_demo}. These attacked images were created using anti-forensic generator trained against Xception.  Visually comparing the GAN-generated images to the attacked images, we can see that there is no visible difference between the two. This demonstrates that our attack will not leave behind visual cues and it will not alter the content of the attacked image in an undesirable manner.

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{figures/face_demo}
\caption{ Attacked images produced by  zero-knowledge attack. }
\label{fig: face_demo}
\end{figure}

\subhead{Comparing with Adversarial Example Attacks}We also compared with performances of CW,  FGSM and PGD attacks.  To measure the transferability of an adversarial example attack against a pariticular victim CNN detector,   we launched the attack against every other CNN detectors,  then used the victim CNN detector to classify the attacked images,  and calculated the mean of the attack success rates.   For a fair comparison,  we chose the parameters for each adversarial example attack such that the mean PSNRs of produced attacked images were on the same level as our proposed attack,  and then we compared the performances of adversarial example attacks with our proposed attack in terms of mean attack success rates.

From Table~\ref{tab:zeroface} and Table ~\ref{tab:zeroobject},  we can see that on human face dataset none of the adversarial examples can transfer to fool CNN detectors,  and on object dataset,  these attacks demonstrate  some transferabiliy  and PGD performed the best among the three attacks with $0.5947$ attack success rate.   Comparing with our proposed attack,   the proposed attack can uniformly fool CNN detectors on both datasets with a  significant higher attack success rate. 







==> sections/zero_results_v1_icpr.tex <==
%zero knowledge results

Table~\rom{3} shows the  performances of attacks achieved on both datasets in white-box scenarios.   Each entry in the table corresponds to the mean attack success rates and mean PSNR  achieved by an attack when attacking a particular victim CNN detector.


\subhead{Human Face Dataset Attack Success Rates} 
The left half of Table~\rom{3}  shows the performances of attacks using the human face dataset.
 On average,  the proposed attack achieved $0. 7510$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of human faces.   While the average attack success rate decreased $15\%$ comparing with  the white-box scenario,   it was mainly because of low attack success rates against ResNet-50 and MISLNet.  We still achieved high attack success rates for the other six CNN detectors. 

\subhead{Object Dataset Attack Success Rates}
The right half  of Table~\rom{3}  shows the performances of attacks using the human face dataset.
On average,  the proposed attack achieved $0.7030$ attack success rate on fooling CNN detectors trained to detect GAN-generated images of objects.  We note that the drop on the average attack success rate comparing to the white-box scenario was mainly caused by SRNet and MISLNet.  We still achieved high attack success rates for the  other six CNN detectors.  

\subhead{Interpretation of the Results}The attack success rates achieved on both datasets demonstrate that the proposed attack can  transfer to fool CNN detectors even when the attacker has zero-knowledge about the CNN detectors.  The results are important because it shows that our attack can be launched in a realistic scenario.  While the results are not perfect,  particularly in the attacks  against  ResNet-50 and MISLNet on the  human faces dataset and the attacks against MISLNet and SRNet on the object dataset,  the results still strongly show that the proposed attack can pose enough threat,  since it worked  great on the majority of the testing cases.  For example,  the attack success rates against Xception are uniformly high (over $0.90$) on both datasets.  
One possible explanation for the low attack success rates in some cases could be that  forensic traces learned by these victim CNN detectors are not located in the same feature space as the ensemble of CNN detectors used to train the attack.   However,  we think it may provide some insights for the investigators and researchers  developing  defense strategies against similar types of attack. 


\subhead{Visual Quality} 
The average mean PSNR  is $40.46$dB  for the human face dataset and $41.27$dB for the object dataset.  These results show that  the attacked images produced by our proposed attack can maintain very high visual quality. 
%The right sections of Table~\ref{tab: zeroface} and Table~\ref{tab: zeroobject} show the evaluation of the image quality of attacked images produced by the proposed attack.    On the human face dataset,  the average mean PSNR is $40.46$ and the average mean SSIM is $0.9682$.  On the object database,  the average mean PSNR is $41. 27$ and the average mean SSIM is $0.9456$.  

We present attacked images of human faces produced by the proposed attack  in Figure~\ref{fig: face_demo}. These attacked images were created using anti-forensic generator trained against Xception.  Visually comparing the GAN-generated images to the attacked images, we can see that there is no visible difference between the two. This demonstrates that our attack will not leave behind visual cues and it will not alter the content of the attacked image in an undesirable manner.

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{figures/face_demo}
\caption{ Attacked images produced by  zero-knowledge attack. }
\label{fig: face_demo}
\end{figure}

\subhead{Comparing with Adversarial Example Attacks}We also compared with performances of CW,  FGSM and PGD attacks.  To measure the transferability of an adversarial example attack against a pariticular victim CNN detector,   we launched the attack against every other CNN detectors,  then used the victim CNN detector to classify the attacked images,  and calculated the mean of the attack success rates.   For a fair comparison,  we chose the parameters for each adversarial example attack such that the mean PSNRs of  attacked images were on the same level as our proposed attack.
% and then we compared the performances of adversarial example attacks with our proposed attack in terms of mean attack success rates.

Table~\rom{3} shows that on human face dataset none of the adversarial examples can transfer to fool CNN detectors.  On object dataset,   adversarial examples attacks demonstrate  some level of transferabiliy,   and PGD still performed the best  with $0.5947$ attack success rate.   However,   our proposed attack still achieved more than $10\%$ higher attack successful rate tha PGD.  Additionally,   the proposed attack cna uniformly fool CNN detectors on both datasets. 






